Protecting File Activities via Deception for ARM TrustZone

A TrustZone TEE often invokes an external filesystem. While filedata can be encrypted, the revealed file activities can leak secrets. To hide the file activities from the filesystem and its OS, we propose Enigma, a deception-based defense injecting sybil file activities as the cover of the actual file activities. Enigma contributes three new designs. (1) To make the deception credible, the TEE generates sybil calls by replaying file calls from the TEE code under protection. (2) To make sybil activities cheap, the TEE requests the OS to run K filesystem images simultaneously. Concealing the disk, the TEE backs only one image with the actual disk while backing other images by only storing their metadata. (3) To protect filesystem image identities, the TEE shuffles the images frequently, preventing the OS from observing any image for long. Enigma works with unmodified filesystems shipped withLinux. On a low-cost Arm SoC with EXT4 and F2FS, our system can concurrently run as many as 50 filesystem images with 1% of disk overhead per additional image. Compared to common obfuscation for hiding addresses in a flat space, Enigma hides file activities with richer semantics. Its cost is lower by one order of magnitude while achieving the same level of probabilistic security guarantees.

==> abstract.tex <==

\begin{abstract}

A TrustZone TEE often invokes an external \fs{} for data storage. 
While the data can be encrypted, the revealed file activities may leak TEE secrets. 
To hide the file activities from the \fs{} and its OS, 
we propose \sys{}, a deception-based defense in which the TEE injects sybil file calls as the cover of the actual file calls. 

\sys{} contributes three new designs. 
(1) To deceive a knowledgeable OS, the TEE generates credible sybil calls by replaying segments of file calls from the very code under protection. 
(2) To make numerous sybil calls low cost, 
the TEE isolates a physical disk and exposes $K$ virtual disks, only one of which is used as actual. 
On the $K$ virtual disks, the TEE requests the OS to instantiate $K$ \fs{} images. 
Keeping the OS oblivious, 
the TEE only runs the actual \fs{} image on the physical disk; it emulates disks for all sybil images by only storing metadata but discarding filedata, reducing their overhead by one order of magnitude. 
(3) 
To protect the \fs{} image identities, 
the TEE renames them frequently and efficiently, preventing the OS from learning long history of any image. 


We implement \sys{} and test it on unmodified \ext{} and \ffs{}. 
On a commodity Arm SoC, the TEE can concurrently run as many as 20 sybil \fs{} images with only 2.2$\times$ slowdown in file accesses. 
Compared to existing hiding techniques such as data shuffling and padding, \sys{} achieves practical protection while reducing the overhead by two orders of magnitude. 


 













\end{abstract}



==> algo-fsnr.tex <==
\begin{algorithm}
	\SetAlgoLined
	\KwIn{
		
		$f(i, B, M)$: all filesystem images;
		
		$T$: maximum tolerable period/exposure window;
		}
	\KwOut{$f'$: new set of filesystem images}

	return S\;
	\caption{\code{fork\&rename}}
	\label{algo:fsnr}
\end{algorithm}

\begin{algorithm}
	\SetAlgoLined
	\KwIn{
		
	}
	\KwOut{ret: xx }
	return ret\;
	\caption{\code{retire}}
	\label{algo:retire}
\end{algorithm}



==> algo-obfuscate.tex <==

\begin{algorithm}
	\SetAlgoLined
	\KwIn{
		
		$f$:the real fs call issued by the secure app in SW;
		
		s: file name of the file to be accessed;
		
		flag: the flag passed to the fs;
		
		}
	\KwOut{S: an array of obfuscated fs ops}
	
	$S \gets \emptyset $\; $i \gets 0 $\; $n \gets 0 $\;
	\If{$f$ is \code{open()} or \code{close()}}
	{
		\For{i = 1 to \K{}}
		{
			S.append($f$)\;
			
			/* create \K{} - 1 buddy files */
			
			/* \note{May detect the existence of buddy file by table lookup} */
			
			\If{flag \& O\_CREAT and i < K} {
				/* persistent binding */
					
				generate random name for buddy file  $s_i$ and \note{bind} $s_i$ with $s$ \;
			}
			
		}
		return S\;
		
	}
	total\_ops.add($f$)\;
	draw $i \sim \mathcal{U}(0, \K{})$\;
	\For{0 to i}
	{
		draw $n \sim \mathcal{U}(0, total\_ops.size())$\;
		S.append(total\_ops[$n$])
	}
	return S\;
	\caption{\code{enigma\_obfuscate()}}
\end{algorithm}


\begin{algorithm}
	\SetAlgoLined
	\KwIn{
		
		$f$:the real fs call issued by the secure app in SW;
		
		s: file name or file descriptor of the actual user file to be accessed;
		
		flag: the flag passed to the fs;
		
		sz: read/write size
		
	}
	\KwOut{ret: return results of the real fs op}
	$ret \gets 0$ \;
	$S \gets \code{enigma\_obfuscate(f, s, flag)}$  \;
	Shuffle the fs op order of S\;
	\For{each buddy file $s_i$ of user file $s$}
	{
		\For{each fs op $f'$ in S} 
		{
			/* avoid appending to the real file system */
			
			/* \note{should work with all ops that do not change metadata} */
			
			\If{$f'$ is \code{append()} and $f'$ is not $f$ }	
			{continue\;}
			
			/* execute the obfuscated file system ops */
			
			$ tmp \gets f'(s_i, pad(sz))$\;
			\If{$f'$ is $f$ }
			{
				$ret \gets tmp$\;
			}
		}
	}

	return ret\;
	\caption{\code{enigma\_exec()}}
\end{algorithm}



==> api-eg.tex <==

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstset{emph={%
	VALIDATION, O_UNTRUSTED%
	},emphstyle={\color{red}\bfseries}%
}%



\lstdefinestyle{mystyle}{
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

\lstset{style=mystyle}
\lstset{
xleftmargin=5.0ex,
framexleftmargin=5.0ex,
frame=tb, %
breaklines=true,
numberblanklines=false,
captionpos=b,
numbers=left,
label=list:api}
\begin{lstlisting}[caption= Code example showing the use of untrusted reads. The augmented API is highlighted in bold and red. ,escapechar=!,label={code:api}]
for (i = 0; i < N_FILES; i++) {
	/*Allow read to return untrusted data*/
	fd_in=open(in[i],O_UNTRUSTED|O_RDONLY);!\label{line:open}!
	fd_out=open(out[i],O_CREAT|O_WRONLY); !\label{line:open2}!

	/*Determine data size for read*/
	fstat(fd_in, &stat);
	/*Read untrusted data*/
	ret=read(fd_in,buf,stat.st_size); !\label{line:read}!

	/* Make image */
	img = make_image(buf, IMG_JPG);
	/* Processing untrusted data. slow. */
	ret = detect_license(img, buf, &sz); 

	/*Wait for validation*/
	ret = select(fd_in, VALIDATION, ...); !\label{line:select}!
	if (ret == SUCCESS) { /* validated */
		/* Write results to new file */
		write(fd_out, buf, sz); !\label{line:write}!
	} else { /* validation failed */
	   /*..discard compute results..*/
	}
	close(fd_in);	
	close(fd_out);
}
\end{lstlisting}




==> app.tex <==

\paragraph{Smart device applications}
Atop \sys{}, we build three applications derived from real-world smart devices:
\note{better descriptions of app-specific metrics}

\begin{myenumerate}
	
	\item A \textbf{cleaning robot} (\code{Robot}) for house cleaning~\cite{rev-eng-mi-robot}.
	We derive the workloads from Xiaomi Vacuum Robot~\cite{vacuum-log}.
	When cleaning, the robot sequentially updates a log file every 200ms;
	each entry is 32-byte 3-tuple containing coordinates (x, y) and the angle. 
	After cleaning, the robot reads back the whole log file, reconstructs the cleaning map using SLAM in PPM format; each pixel of the map is 5cm in physical world and a typical map size is therefore tens to a few hundred KB.
	At last the robot writes back the map file to disk.
	We fix the log size to 512KB and map size to 256KB.

	
	
	\item A \textbf{voice assistant} (\code{Voice}) for interacting with user speech commands~\cite{mycroft}. 
	We derive the workloads from Mycroft~\cite{mycroft}.
	When starting, the voice assistant first loads a set of user-defined rules, called \textit{skills}, to respond to user speech;
	each skill is a directory under \code{\textasciitilde/.mycroft/} containing a \code{.voc} and a \code{.intent} file to identify the intent of user, a \code{.dialog} file to respond to user, and a \code{.json} file to describe the skill;
	every 2s the device will scan the three skill files using \code{fstat} in case any modification or updates.
	After boot, it listens to the user speech in the background, records the audio, and stores the recording as a \code{wav} file under \code{/tmp}; 
	it then runs speech to text transcription (STT) and responds to user according to the STT results and existing skill.

	\item An \textbf{intelligent camera} (\code{Camera}) for license plate recognition.
	We derive the workloads from intelligent traffic systems.
	As the surveillance goes on, the camera periodically captures and saves images (1080P in JPG format).
	Every other 10 seconds, it reads in the saved images and runs license plate detection algorithm on them;
	on the images, the algorithm detects canny edge, dilates them, and then find license plate blobs.
	Finally, it draws bounding box around detected plate blobs and saves the resulting image.
	We use images from UFPR-ALPR dataset~\cite{ufpr-alpr}.
	For the application, we ported to TEE \code{SOD}~\cite{libsod}, a popular embedded computer vision library.
	
\end{myenumerate}

	These applications serve as our macrobenchmarks. %


==> assumptions.tex <==
\subsection{Assumptions}

execution characteristics, fs behaviors, etc.

==> benchmark.tex <==

\subsection{Kernel microbenchmarks}


==> benchmarks.tex <==

\subsection{Microbenchmarks}

\Paragraph{Benefit of energy efficiency}

==> design-choice.tex <==
\subsection{Design space exploration}
\note{then given previous arguments, this section mainly explore design space under two assumptions 1) cloud-local pair is needed, 2) replicated execution is needed}



In this section, we explore the design space for cloud-backed file systems and then present our choice.
























\label{sec:exploration}


\paragraph{What \textit{least} knowledge does cloud need?}
In designing such a distributed file system whose major goal is to provide aforementioned strong security guarantees, we keep the question in mind: \textit{what least knowledge does cloud need}, because even though the cloud is a must to achieve our security goals, we still want to minimize the potential attack surface.

To answer this question, in Figure~\ref{fig:spectrum} we lay out a broad spectrum of networked systems based on how much knowledge the cloud has (i.e., how data and metadata is replicated).
On the bottom left sits the systems \cite{cfs} where neither metadata nor data is replicated and there is \textit{only} one copy of metadata and data, as exemplified by a networked file system (e.g., Linux NFS). 
On the top left sits distributed file systems~\cite{coda,dropbox}, where the cloud and local side keeps distinct metadata themselves and only data is replicated to the cloud.
The top right includes remote execution systems~\cite{clonecloud,maui} that replicate all the metadata/data on both the local device and the cloud, which also often replicate all file operations on both sides. %

Almost all prior systems replicate user data to the cloud.
In contrast, we argue to avoid so for securing IoT file systems, 
because i) we do not necessarily entrust the cloud for user data confidentiality~(\S\ref{sec:bkgnd:security}),
and ii) the network bandwidth, especially that of uplink, is limited~(\S\ref{sec:backgnd:rationale}).





\begin{figure}[t!]
	\centering
	\includegraphics[width=0.35\textwidth{}]{./figs/design_space} 
	\vspace{5pt}		%
	\caption{The design space for cloud-backed file systems, plotted based on how user data and metadata are distributed.
	}
	\label{fig:spectrum}
	\vspace{-10pt}		%
\end{figure}



\paragraph{Our design point}
\note{should be tied to security and talk less about performance}
Towards securing IoT file systems, we advocate replicating only the metadata but not the user data to the cloud, as shown in the bottom right part of Figure~\ref{fig:spectrum}. 
As a result, the cloud executes a \textit{metadata-only} file system replica, and is able to validate the legitimacy of any data operations to be performed on the IoT device, defeating \textit{Iago attack} caused by delegating file operations to the commodity file system. 
By avoiding replicating the user data to the cloud, we avoid trusting the cloud for user data confidentiality or integrity as there is no data at all. %

























 


























==> design-disk-migrate.tex <==
\section{Continuous filesystem name randomization}
\label{sec:design:fsnr}


\textbf{A key defense} is to limit observation period. 
Why is this important? There are two reasons. 

\begin{myitemize}
\item 
(exposing long history is risky -- capability of reasoning about \fs{} long-term behaviors. More powerful to break the camouflage and identify the actual \fs{}. 

\item
(coping with accidental exposure) 

Despite the efforts in making sybil \fs{}s indistinguishable from an actual \fs{} through trace record-and-replay, the identity of actual \fs{} may eventually be exposed due to unexpected channels.
E.g. the distribution chosen by the trustlet does not conform to an actual one. Once the OS identifies the true \fs{} successfully, it reveals full history of actual file traces (assuming the OS is computationally unbounded)
\end{myitemize}

\textbf{Key observation -- \fs{} image identities}
How do the OS identify/track a \fs{} image? Either of two pieces of information:
1. a \fs{} image's binding to underlying block device. (obvious)
2. a filesystem's metadata that is exposed to the OS (non obvious)

\textbf{Idea}
In a nutshell, FNSR swaps (renames) \fs{} images with identical metadata -- in an oblivious fashion to the OS. 
Users specify a maximum tolerable period $T$ for continuous observation. 
\sys{} ensures that the OS can only track the identity of any \fs{} image F (sybil or actual) for a continuous period no longer than $T$. 
Why doing so to sybil? Because egalitarian principle. 

\sys{} takes one of two possible actions: 
it shuffles (renames) underlying block devices for \fs{}s that have identical metadata oblivious to the OS; 
or, it forks F and creates new \fs{} images with identical metadata. 
The two mechanisms render the OS incapable of pinpointing which of the resultant \fs{} image (as outcome of renaming/ is $F$.

The results are twofold: 
1. the OS cannot establish a history of any \fs{} (including the actual fs) longer than $T$;
2. in case of accidental identity exposure, the OS can only exploit it for no longer than $T$ before the next round of FNSR happens. 

\textbf{To retire}
Last but not the least: this happens in the background (async). 
It resembles GC -- to collect excessive \fs{} images. 
Corollary: 
	any \fs{} (actual or sybil) can be forked and renamed. 
	only a sybil \fs{} can be retired. This has strong implication on protection. See below. 
	
This resonates with moving target defense (MTD) to make it harder for the attacker to keep track of actual fs; 
These echo with the motivations of continuous ASLR, which deal with program address space while we deal with filesystem namespace (i.e. actual vs. sybil).
	
\input{fig-fnsr}

\paragraph{Security analysis -- Why this works -- from the OS POV}
Through forking/renaming, FNSR produces an ancestry of \fs{} images (sybil and actual) over time. 
As can be seen from the figure, 
as a \fs{} image forks, it becomes the ancestor of all resultant \fs{} images. The OS cannot continue its (forward) tracking.
After a set of \fs{} images participate renaming (shuffling), 
they all become \textit{probable} ancestors of the resultant \fs{} images. 
This is because the OS does not know the renaming (shuffling) scheme. 
The OS is unable to track (forward and backward) of \fs{} images. 

The OS knows: the entire topology of ancestry as the complete history of FNSR. 
Being computationally unbounded, the OS memoizes the history and will use it to uncover the actual \fs{} images. 
			
\subsection{Algorithm sketch}

(could go to a code listing)

\input{algo-fsnr}

\begin{myitemize}
\item Keep an ``exposure'' timer. 
The timeout is user-defined maximum exposure. 

\item Whenever a timer for fs $F$ expires: 
	Check for renaming opportunities. 
	
	\begin{myitemize}
	\item 
	Do other fses have same metadata as $F$? If so, rename them opportunistically. 
	
	\item 
	If not, fork $F$ into multiple (how many?) \fs{} images. 
	
	\end{myitemize}

	Reset the exposure timers for all participating fses. 
	
	\item Retire ...	
\end{myitemize}
			
\Note{Challenges and solutions}

\textbf{Challenge: backtrack Attacks}
The root reason is that only sybil images, but not the actual image, can retire. 
The OS could exploit this invariant. 
From all of the currently alive \fs{} images, the OS could trace back to their probable ancestors and rule out sybil images earlier in the history (since they retire, they cannot be the actual \fs{} images). 

(through backtracking) if in an earlier generation the probable ancestor are fewer than K, the (K anonymity) targeted (promised) by \sys{} is weakened. 
In an extreme case, if in an earlier generation there is only one probable ancestor F, the OS knows F must be an actual image. 

A successful adversary that identifies F as the actual \fs{} image in generation G could uncover a segment of actual file trace: from G, the OS further backtracks F's ancestor images until the most recent renaming (shuffling) point; the OS forward tracks F's offspring until the subsequent forking/renaming point. 
During this period, the OS is certain that F is \textit{the} actual image. 
Hence, all the actual ops done on F between the two points are exposed. 


\textbf{Solution:}
When \sys{} picks a \fs{} image to retire. 
It only retires a \fs{} image if the would-be probable ancestors in any of the previous generation is no fewer than K. 
\sys{} determines the probable ancestors by backtracking just as the OS would do. 
Must respect the above invariant when we choose \fs{} images to delete/retire. 




\textbf{Challenge: too many \fs{} instances?} 
Will respecting the above invariant make \sys{} incapable of retiring \fs{} images, leading to excessive \fs{} images? 

This will not happen for two reasons.

1. At a generation G there are S images that come from K \textit{probable} ancestors in all previous generations. 
As long as S > K, there is at least one image: after retiring, the set of probable ancestors in G-1 is unchanged. 
Therefore, the set of probable ancestors in G-2 is also unchanged...

(do we have to consider the age of the image to retire? That is, if it is newly forked, we should not retire it?)



2. In practice, forking does not have to be often. 
Many \fs{} images (sybil or actual) have the same metadata. 
The reasons: ops that change metadata are (relatively) sparse (??); 
actual/sybil \fs{}s are produced by traces from the same trustlet. 
In many cases the difference is only the replay rate. 
Example: video surveillance trustlet - regular append only pattern. 
Example: queries over db files (read only access) 



\textbf{Challenge: the cost of forking/renaming -- Physical implementation}
We use COW for \fs{} images as backed by our BTT.
Forking/renaming become cheap. 

\textbf{Rename}: 
randomly rebase them on different hosting block devices.
the \fs{} is given a different host block device exposed to normal world, 

phys implementation -- BTT ops: swap the "bdevid" of the two \fs{}s.	

\textbf{Forking}:
replicates existing \fs{}s onto newly registered block devices or the old ones; 
For example, \sys{} replicates a \fs{} image F on block device 1 onto a newly registered block device 2 to form \fs{} image F'.
Then it rebases $a'$ on block device $1$ and $a$ on block device 2. 
From the normal world PoV, the secure world registers a new block device and remounts both \fs{} images.
Afterwards, the normal world OS sees two identical \fs{} images (i.e. F and F') but is uncertain if F is still on device 1.

\textbf{BTT ops:} inserting rows w/ new sbd sectors while having same \backend{} sectors as the replicated \fs{}.

\textbf{Retire}: this deletes entries in the metadata store. 		
the \fs{} is dropped/recycled from its block device. drop all entries belong to "bdevid".
	
 

 







==> design-disk.tex <==
\section{Backend: \sys{} secure backstore}

\sys{} partitions the commodity storage stack -- while leaving/reusing all \fs{} implementations outside \tz{}, it pulls the storage device into \tz{} to form \sys{} secure backstore, as discussed in Section \ref{sec:overview:idea}.
Doing so enables \sys{} to fully own the storage device (thus system metadata) in \tz{}.
More importantly, it facilitates \sys{} to mediate block-level access between storage and \fs{}s, a key enabling factor towards obfsucation transparency and efficiency -- it maintains the ``illusion'' of sybil \fs{}s by covertly dropping the respective block ops of injected ops and ensuring the same timing as the actual \fs{}.%

In this section, we first describe secure data path where trustlets interact with \fs{}s and secure backstore, to give an overview workflow of the partitioned storage stack design.
Under such design, we then describe \sys{}'s block-level access rules and time protection mechanism for maintaining the sybil \fs{} illusions.


\paragraph{Overall goal}
Low storage cost (through aggressive opt - drop the storage ops on sybil fses) while maintaining confidentiality (meaning identity of the real fs?).
\note{use the ``mediate'' block level access}

Two noteworthy designs: access rules \& time protection.





















\subsection{Overall workflow: secure data path}

\sys{}'s secure data path (Figure~\ref{fig:arch},  \circled{4}) resembles a trusted IO path\note{cite}, whereas user data flow, device drivers all run inside \tz{}, without going through the normal OS.
However, it is only ``semi''-trusted since the \fs{}s are left outside \tz{} instructing the execution of secure data path.
\Note{cite previous work, share the spirit of trusted io path, ... with a key diff...}

This is a natural design choice we put the storage inside \tz{} since the trustlets own both the data source/dest buffers as well as the disk. 
Data move due to trustlet r/w directly happens within the tz, going from the buffers in the trustlet to the secure storage.  
More importantly, it facilitates the "cover disks" that makes sybil \fs{}s practical.



It works as follows:

\Note{replace ``buf addr'' with opaque ref, which is just to hide the tz addr from the OS (to avoid info leakage). note that we do not protect against ref fabrication which is out of the scope of a curious OS} 

\begin{myenumerate}
\item the obfuscator (\circled{1}) forwards the obfuscated file trace. 
For data buf addr of all file ops (e.g. \code{buf} field in examples in \S~\ref{sec:motiv:case}) in the trace, \sys{} passes one \tz{} buf addr.

\item 
the \fs{}s (\circled{2}) receive the file ops, execute all, and produce a bunch of block requests;
\fs{}s then submits them to the secure backstore.
By design, the submitted block reqs preserve the buf address -- block req to operate on data (i.e. data block req) has \tz{} addr; block req to operate on metadata (i.e. metadata block req) has NW addr.

\item 
the secure backstore (\circled{3}) receives them (block requests) but only executes those from the actual \fs{} and from metadata block req in a sybil \fs{}. 
It silently drops data block ops for sybil \fs{}es. 
This is completely transparent to the OS.

\item 
Block data req of the trustlet directly interact with the storage (pull data block to the buf addr or write data inside buf addr to disk blocks) -- this is secure data path (\circled{4}).
Figure~\ref{fig:arch} shows the secure data path in a block read scenario.

\end{myenumerate}




\subsection{Secure against the OS -- maintaining the illusion}


\paragraph{The illusion of sybil \fs{}s}
While only data block reqs of actual file ops and meta block ops are executed, data block reqs from injected dummy file ops are \textit{covertly} discarded (see above).

This creates an illusion of sybil \fs{}s:
they are \fs{}s running with only metadata;
the metadata still bookkeeps data block allocations without knowing the data blocks do not exist on the disk.

This is also the key to low cost (our design challenges in \S~\ref{sec:intro}) and to maintaining $K$ \fs{}s for the sake of obfuscation: 
1. transparency -- covert, without \fs{} knowing (we own the device);
2. low execution overhead -- no actual block ops;
3. low storage overhead (metadata vs data).
 

To maintain such an illusion, \Note{for fs to operate properly... (perhaps this shall be stated upfront)}
\tz{} needs to serve metadata to the \fs{} (both actual and sybil) .;
it therefore must respond to metadata block req of the fs, allowing the disk to read/write them.
This is because for a \fs{} to operate properly, it must read, modify, and update the metadata (e.g. inode) that is stored alongside the user data on the disk. 
What is more, these reqs must be responded properly: 
on one hand, it must allows those with a nw address since they are metadata block req;
on the other hand, it must not leak user data while convincing the OS that user data exists (i.e. not sybil).
\paragraph{Challenges}
To summarize, the challenge is while the secure storage must allow disk writes and reads from the \fs{}s \Note{does this mean r/w metadata?}, 
it should maintain the illusion to a curious \fs{} that all the sybil storage devices indeed exist as an actual \fs{} both in ``material'' and in ``time'' (without actually allocating/maintaining the blocks?)

\Note{The challenge is not trivial...}
Unfortunately, per our threat model, a malicious block read can happen to break user data confidentiality and the camouflage of a sybil \fs{};
attack vectors are listed below.

\Note{why do we care about leaking user data which is encrypted? we shall only care about revealing which fs is actual}

\paragraph{1. Rogue read to data blocks}
The attacker uncovers user data by forging a metadata block req, which comes with a nw buf addr but directs to data blocks. %
Since \tz{} has no \fs{} knowledge, it cannot decide if the req is indeed a metadata block req that keeps \fs{} running; 
hence it has to allow the req to happen, which results in user data leakage. \Note{can be gone}
Similarly, the attacker may direct the forged metadata block req to data blocks of a sybil \fs{}. 
The attacker may reveal its identity (i.e. sybil) by figuring out they do not have any data blocks (and that previous writes are ineffective).
That is, if \tz{} feeds the OS with arbitrary data 
when the OS requests to read these ``non-existent'' data blocks, it may find out two back-to-back reads of the same block returns different values!
\Note{tz cannot return fabricated data that is randomly generated on the fly}

\paragraph{2. Leveraging block timing side channel}
\Note{describe the OS/TEE interactions; how OS could measure the timing; two ways to mount the attacks}

\begin{myitemize}
\item sybil data blocks do not exist
\item metadata layouts are so different 
\end{myitemize}

Besides reading from the block content (i.e. the above), block timing side channel is also at attacker's expense to poke the existence of a sybil \fs{}. 
Since sybil \fs{}s only have metadata, it does not make sense to pan them out to own a full partition (which we also try to avoid for the sake of storage) like an actual \fs{} does;
as a result, the different block locality of sybil \fs{}s from an actual \fs{} may eventually result in timing differences at block reads.
``their illusion'' does not instantiate into a full physically-existent \fs{}.


We will address the above challenge in the next sections.




\subsubsection{Access Rules: Blocking Rogue Reads}

\Note{we do not consider inline (data/metadata coexisting), why? justify it}

The root cause of a rogue block read is: without \fs{} logic, \tz{} lacks block access control. 
\note{the below is only to show a strawman policy and that our access rule is not as trivial}
\Note{It just shows that static distinction does not work, right? Dynamic tracking seems not a key idea}
To remedy and devise access rules, one may leverage metadata vs data block distinction and only allows access to metadata blocks.
At \fs{} creation time, \tz{} keeps track of all blocks being written, marks them as metadata blocks, and grants only access permission to normal world OS on them.
The one-shot efforts work for ext family when metadata blocks are statically allocated -- a physical block is bound to store metadata or data. 
This, however, does not work for other \fs{}s which have dynamic metadata blocks (e.g. log-structured \fs{}s) -- blocks can be recycled/GCed at runtime to host metadata block or data blocks, where \tz{} has no knowledge of. 
\Note{the role of blocks are mutable at runtime}

\paragraph{Our key idea}
\note{if we donot need a strawman design above we can delete the transitioning sentence}
Compared to a ``static'' rule which fails to track the dynamics of a \fs{}, our observation is intuitive: 
\begin{myitemize}
\item 
All metadata is generated by the \fs{} and thus the secure storage should allow the \fs{} to access.
\item 
All data originated in the \tz{} is user data that should not exposed to  the \fs{}. 
\end{myitemize}

Therefore, as data is written from the beginning, \tz{} tracks block ownership state\note{may need a better term or change the current one?} (\fs{} vs. \tz{}) and enforce the following access rule. 

\Note{what's the rationale?} Only materialize a block (i.e. physically allocating it on disk) when it gets exposed to the \fs{}. 

\input{fig-block-access-rule}

\paragraph{Access rules}
We summarized the access rule in a state transition diagram shown in Figure~\ref{fig:block-access-rule};
upper left triangle is the state transitions allowed on blocks storing sybil filesystem;
lower right triangle describes block state transitions in an actual filesystem.
Details of the access rule follows:
\begin{myitemize}
\item Four ownership states of each block -- $\{(un)tainted\} \times \{(un)materialized\}$

\item $tainted$ block is tainted by normal world OS, $materialized$ block is the block with persistent data. 

\item By default, all blocks are untainted/unmaterialized. 

\item Taint a block if the OS ever writes (``untagged'' writes) data to the block.
Materialize a block once TZ writes to it or NW issues a metadata write.

\item 
Semantics of the block states are:

\begin{myitemize}
	\item Tainted \& Unmaterialized: sybil file data blocks \Note{?? why tainted??}
	\item Tainted \& Materialized: meta blocks (or blocks containing metadata) in sybil|actual fses. 
	\item Untainted \& Unmaterialized: unused blocks; \textbf{sybil file data blocks}
	\item Untainted \& Materialized: data blocks in actual fses
\end{myitemize}


\end{myitemize}



We show an example process below, demonstrating both a legal read and a rogue (injected) read trying to revealing user data block/sybil data block.

\Note{the following needs refinement -- see states above}

\begin{myitemize}
	
\item The OS wants to read an unmaterialized block, denoted by the gray triangle in Figure~\ref{fig:block-access-rule}: return 0.
All possible content held on such data blocks: empty (either never allocated or used to hold sybil file data) or actual user data.
This tracks the data originated from \tz{}, as part of our key idea. 
Return 0 == reject == no information leakage.

\item The OS wants to read from a tainted block: give it the actual value. 
Reason: tainted by the OS means the data is originated from the OS (this is our key idea) 
Hence, we deem it a metadata block and allows read.

\item The \tz{} wants to write to an unmaterialized block: write as it should for actual, drop them for sybil \fs{}s. 
This describes a new data block is being allocated to the filesystem used to host data -- for actual do the write and drop those of sybil.


\item The \tz{} wants to write to a tainted block: do the actual write. 
This happens when a metadata block for actual \fs{} is recycled to host data block.
\Note{or metadata and userdata colocated on the same block?}

\end{myitemize}

\subsubsection{Emulating secure storage of sybil \fs{}s}
The key idea is also to separate and separately handle data and metadata requests.

For all data block requests, actual or sybil, \sys{} leverages (1) the existing, commodity modular \fs{}-block design and enforces them to async (to the fs).
This means \fs{}s only submit these requests to secure backstore (in TEE) and return.
This conforms to \fs{}'s original semantics, because 1. (1) by-design specifies an async interface for \fs{} and block device,
2. data req are out of \fs{}'s critical control path, which they do not check completion.
Yet, it blocks the OS's observations on the completion of data requests -- they are fully executed/enclosed inside the semi-trusted IO path.

For metadata block requests, which OS demands to be notified of the completion, \sys{} leverages (2) the fully owned secure storage (again) and notify the OS with ``appropriate'' timing.
For metadata block requests to actual \fs{}, their completion timing is delivered as-is;
for those of sybil \fs{}s, secure backstore adopts the well-known idea~\cite{david} to emulate a ``compact'' \fs{} (i.e. sybil).
It adopts a storage performance model to capture the precise timing of these requests being executed;
according to the model, it injects delay before notifying the OS, which is also adopted in previous work~\cite{time-protection}.
Why always delay? This is because sybil \fs{} by design is way more compact (only metadata, no data) than an actual \fs{} -- block req is always faster on sybil \fs{}s.


--------------


Our goal:
1. To hide the fact that a sybil \fs{} contains actual data blocks when being probed.
2. To hide the fact that sybil \fs{} metadata exists as ``sparse'' as an actual \fs{}.

Attack vector: OS reads a data/metadata block of a sybil \fs{} and measures its access time.

Approach: storage model, similar as David\note{cite}. 
Inject delay based on model output.
This is for outstanding block read. 

Q: how to hide that sybil block req are dropped?
Q: what is the max degree of concurrency for mmc? how many mmc req can overlapped simultaneously?

A simple solution seems to break part of the semantics of the original fs -- directly notify completion of ALL data requests (actual and also sybil) and does not break that of meta requests (w/ latency injected to sybil \fs{} meta requests).





\Note{To write:}
We inject delays to access of nonexisting data and to access of metadata that exists. 
The problems are existing/nonexisting and locality. Can we solve with some simple strategy? 

Todo: look at disk/storage performance modeling work. 

\begin{myitemize}
	\item approach -- modeling? 
\end{myitemize}




\subsubsection{How do they thwart aforementioned attacks?}
First, recall how it works in a normal process as described above.
Recap the attacker's capability -- passive, honest-but-curious; it does arbitrary reads but only ``legit'' writes.

Then, consider an attack scenario, where the attacker tries to read blocks from the disk to decide if they host actual/sybil files.

\begin{myitemize}
\item 
write dir blocks \Note{why care about dir blocks? just as example meta blocks?}, read back -- allowed, they are tainted and materialized and the block content will be returned as-is.

\item 
write metadata blocks, read back -- same as above.

\item 
directly read back file blocks -- sybil file blocks are unmaterialized, actual file blocks are untainted, both will return 0 -- cannot differentiate which is which.

\item 
wants to write to file block and read back -- only happens to LFS but not ext due to GC. 
We support this -- both tainted/unmaterialized and untainted/materialized blocks will be materialized into tainted/materialized blocks (data block -> metadata block).
Read back will get previously written content, because the blocks are materialized.
\Note{need discussion}

\item 
wants to write arbitrary blocks (w/ untagged write) and tries to materialize all of them? 
FS integrity issue, leave it to future work/complementary approach can address.
\Note{out of scope}

\end{myitemize}

The sybil and actual storage partitions will exhibit the same behaviors from the OS POV. 
If the OS ever writes to a block, it reads back what it has written; 
if the OS reads from a block that it never wrote to, it gets 0; 
if the OS reads from a data block of a sybil file, it gets 0;
if the trustlet writes to the same block, the OS reads back, only to see 0.

Note that the access rule is based one key assumption -- the attacker does not do rogue write.



\subsection{Physical implementation}

\subsubsection{Managing sybil file systems}

To eliminate storage overhead of file data, we exploit the key observation that a \fs{} only relies on metadata but not data (\S~\ref{sec:overview:idea}, O2), which only depends on the following two key data structures.



\paragraph{Block req mediator}
A layer of indirection to mediate all submitted block requests.
It does the access rule checking first, if passed will translate it (i.e. a logical block request) to a physical block req on a storage.
It also handles block allocation. 
For metadata materialized at creation time, it linearly map then to disk (same as an actual \fs{}), for later blocks it reserves a pool and does sequential allocation.
It bookkeeps all the logical->physical mapping of each sybil \fs{}.


\paragraph{Metadata blobs.}
The necessary metadata to describe a \multifs{} and to facilitate it to perform disk block management (e.g., block allocation and retrieval) forms a metadata blob for the \multifs{}.
It stores \textbf{only} the metadata of the \multifs{} compactly as a binary blob.
The metadata blobs differ with respect to individual \multifs{}s. 
For example, \code{FAT} \fs{}'s metadata blob simply contains its super block, and the file allocation table while for \code{ext4}, in addition to super block, its metadata blob also contains group descriptors, data block and inode bitmap, etc.
When operating, access to logical metadata blocks will then be translated to a block within the metadata blob.
It is an inverse analogy to the concept of virtually contiguous but physically discontinuous memory addresses, where in this scenario the (in general) discontinuous logical metadata blocks will be translated to blocks in physically contiguous metdata blob.

\paragraph{The directory pool.}
By operating solely on the metadata blobs, the \multifs{}s lack support for directories.
To remedy this and to enable dynamic directory creation, we introduce the shared directory pool.
The rationale is directories are nothing but normal files of predefined formats and size (i.e., 4KB) hence can be managed centrally.

The shared directory pool is a pre-allocated data file.
Its only responsibility is to allocate data blocks for the \multifs{}s to store directories.
It takes a simple sequential allocation \note{log-structured?} strategy: whenever a \multifs{} requests data blocks to create directories (e.g., on a \code{mkdir}), \sys{} scans the pool sequentially for available blocks and supplies them when found.



\subsection{Putting it together: supporting sybil filesystems and ops with \sys{} secure backstore}
\label{sec:backend:workflow}
Despite managing \multifs{}s with metadata blobs and a shared directory pool avoids file data storage overhead, however, a central challenge is how to \textit{fool} the commodity \fs{}s (i.e., no code modification) such that they can still operate normally while remaining oblivious to the outcome of the data blocks (i.e., whether they are actually stored or not).

To address this challenge, our key insight is to exploit the observation that \fs{} operates on storage data through a narrow, unified block interface (\S~\ref{sec:overview:idea}, O3).
To this end, we partition the storage stack at block interface, leaving the \fs{} in normal wold, and pulling the below part into the \tz{} to form \sys{} secure backstore.


\paragraph{Overview.}
The \sys{} secure backstore (\circled{3}) consists of a block layer and the storage device layer.
The block layer connects the secure backstore with the \fs{}s in normal world by exposing a very narrow message-passing interface -- a command identified by request type (read/write), \textbf{logical} block number, and a buffer address to hold the block data;
the storage device layer then executes the command -- to move data and metadata between the buffer memory address and a block on the storage device.

\paragraph{Supporting \multifs{}s.} \sys{} backstore allocates separate partitions to store the metadata blobs of all \multifs{}s and the directory pool.
The metadata blobs are stored back-to-back in their partition.
\sys{} keeps track of the disk blocks of each metadata blob, and its corresponding \multifs{} using a metadata lookup table. 
The table is created along with the metadata blob (i.e., on a \code{mkfs}) and specifies the logical block to its disk block mapping.
For efficient lookup, the table is backed by a B+ tree.
\sys{} performs searches on it for each incoming block request from \multifs{}s.
If found, indicating the requested block is a metadata block, \sys{} executes the requests -- writing to disk blocks of the metadata blob or reading blocks to the normal world \fs{};
if not found, \sys{} returns an empty block (for read) or discards the write request.



\paragraph{Storing metadata blobs and directory pools for \multifs{}s}
A subtle question to ask is: \textit{who} should bookkeep the metadata?
Conceptually, the metadata is no different than a regular file and thus can be stored and managed by the real \fs{}.
However, to avoid introducing uninvited garbage and to keep user \fs{} transparent, we deem the metadata blobs must be bookkept independent of the actual user file. 

To this end, we allocate a separate partition to store the metadata blobs of all \multifs{}s.
The metadata blobs are stored back-to-back in the partition.
Analogous to a minimalist \fs{}, \sys{} keeps track of the disk blocks of each metadata blob and its corresponding \fs{}.
The knowledge of the metadata blob->disk block mapping will be used in block translation and discussed in the next section.
To support meta ops while avoiding storage overhead, \files{} of the proposed approach (\S xx) are instantiated on \multifs{}s as \textit{data-less} files.


\paragraph{Handling sybil ops.}
\sys{} secure backstore drops data block requests resulted by sybil ops.
As described in \S~\ref{sec:design:obfuscator}, \sys{} obfuscator injects sybil ops to obfuscates the file access pattern.
These sybil ops contain a \code{buf} address that holds the data -- after being forwarded, the \code{buf} address will pass down to embed in the resultant block requests, as described above.
The address is in \tz{} address space, and is recognizable by \sys{} secure backstore.
Upon receiving these block requests, the backstore silently drops them, avoiding executing the actual block IO, eliminating its overhead while keeping the OS transparent.






==> design-explore.tex <==





==> design-goals.tex <==
\subsection{Design Goals and Challenges}

In presence of the powerful adversaries, \sys{} aims to 1) embrace the strong security properties (i.e., data confidentiality, integrity, freshness and verifiable persistence), and 2) facilitate reuse of commodity file systems on IoT devices.
However, with the two goals, we face the following challenges:
\begin{enumerate}
	\item Beyond forging system call to cause data corruption or leakage, a compromised kernel may conduct controlled side-channel to infer the data.
	\item Reusability can only be achieved by delegating file operations.
\end{enumerate}


==> discussion.tex <==
\section{Discussion: Dealing with Cloud Disconnection}

It's not uncommon for IoT devices to experience poor connection with the cloud.
For such a case, 
we propose two mechanisms for the IoT apps to continue to use \sys{}.
First, the runtime executes the pending, unvalidated data operations. 
For reads, it notifies the app that the return data is untrusted. 
For write, it marks the written pages/blocks as untrusted in case the app wants to read from them later. 
It also checkpoints these pages/blocks in case OFS eventually disagrees on, and rejects the data operations.
Our rationale is to rely on the app's domain method to deal with untrusted data in the face of cloud disconnection.
When the connectivity is recovered, all pending data operations will be validated. 

Second, the runtime allows trusted writes of a limited amount of data even at any time, even when connection is down. 
This is important for system log files. 
To do so, during the file system initialization and the cloud is connected, it creates a fixed-size \textit{emergency} file with pre-allocated blocks.
Since the mapping from file offsets to disk blocks is known, an app can safely execute non-cached write to the file at any moment without validation from the cloud. 
The writes are always trusted. 



==> eg.tex <==
\input{fig-perf-breakdown}
\vspace*{-4mm}
\subsection{A case study of using the augmented API}

\input{api-eg}

\sys{} gives applications an option to access file data before validation arrives (\S\ref{sec:design:memoiz}) and hence hide network latency. 
To understand the entailed programming burden and performance reward, we build a revision of the camera application. 
The application open a series of input image files, runs license detection on them, and write results to output image files. 
In the new version, the application opens input images files by specifying the \textit{untrusted} flag (line~\ref{line:open},~\ref{line:open2}).
When the application reads in images, \sys{} therefore returns the data as soon as the local \fs{} gives the block numbers.
As the application gets the untrusted image data, it computes, and executes a validation barrier (line~\ref{line:select}).
Only on successful validation (i.e. the vision algorithm has executed on a correct input image) will the application write back the processed image (line~\ref{line:write}).
With minor source changes, the application overlaps the vision compute with network delay in validating a \code{read}.

Figure~\ref{fig:app} shows the application latency reduction as the reward from handling the untrusted data. 
With fully trusted read/write, the application incurs 26\% higher latency as compared to a native execution baseline; 
with untrusted read, that overhead is reduced to 8\%. 
Note that, the use of untrusted file access is optional. 




==> eval-plan.tex <==

\subsection{Eval plan}


\paragraph{Comparisons}
\begin{myitemize}
\item 
(insecure) Native. Perf baseline.

\item
K files in one FS (i.e. w/o K fses. The fs is bloated.) 
\textbf{Expectation}: storage cost -- much higher; execution overhead -- moderately higher.
\Note{we do not execute IO ops on the dummy files}

\item
K files in K FS (i.e. w/o secure storage in TEE) 
\textbf{Expectation}: storage cost -- much higher; execution overhead -- much higher.

\item
(ours) K files in K sybil FS
\end{myitemize}

Note all benchmarks are IO bound

\paragraph{Macrobenchmark.}

Provides performance breakdown.

Workloads generated by filebench

\begin{myitemize}
	\item Video server: continuously create new video files and delete old ones 
	\item Web server
	\item SQL Lite(Oltp workloads)
\end{myitemize}

\st{ML workloads: YOLOv3} 


\Note{question to answer: zoom into individual file access cost; latency of individual ops}

\paragraph{Microbenchmarks.}
IObench -a -g 1024 -I: auto mode, measure the performance of sequential/random read/write of a single file.

Compare: insecure, w/ sybil fs, w/o sybil fs
FSes: ext4, f2fs

Variable: K

2 rows X 4 cols: each row is an op to an fs, x-axis is K, y-axis is throughput

This is to show as K grows, the overhead grows insignificantly



==> exp-old.tex <==
\section{Early Experience}

\paragraph{Platform}
target platform: omap4, pandaboard. We chose the platform because of XXX. 

Other viable platform: NXP, Beagleboard X15, etc...

\paragraph{Software stack}
Host OS -- Linux 4.4 

Weak core: 
we have already implemented these features... heterogeneous -- for cross ISA execution...

\paragraph{Bootstrapping}

also talk about virtual page setup, carveout memory, etc.

\paragraph{MMU emulation}

\paragraph{DBT engine}
lines of code, etc.

One major challenge is the complexity of DBT engine.

POSIX, strip down existing DBT engine.

Built atop QEMU, We have successfully run a tci backend that essentially interprets the IR. 
The efficiency can be low though, about XXX.
We are building another backend based on ARMv7m (or even ARMv6m). 

We were assuming a clean kernel API (that at least survive across multiple major kernel versions). 
It is hard though, because data structures are passed through the kernel API; and depending on the kernel configuration, the layout (and members) of these data structures can vary differently. 



==> exp-setup-bak.tex <==

\input{fig-exp-setup}
\paragraph{Test setup.}
We test \sys{} on Hikey~\cite{hikey}, an ARM-based development board, as the smart device. 
We choose this board for its good support for \tz{}. 
The details of Hikey are summarized in Table~\ref{tab:plat}. 

\Note{comparisons}
We test \sys{} with \ext{} and \ffs{}, two modern \fs{}s popular among commodity smart devices. 
We run a suite of macrobenchmarks and microbenchmarks. 
Prior to each run, we reboot the device in order to have a cold cache.
We compare with aforementioned two alternative backend designs described in \S~\ref{sec:design:buddy}: 
1) \textbf{K-FS} -- \K{} \files{} are deployed on \K{} \fs{}s and their block requests are executed, 2) \textbf{K-Files} -- \K{} \files{} are deployed on the same \fs{} of the actual user file but block requests of \st{sybil ops are dropped}. 

\note{Why turn off pagecache?}
This is to 1) benchmark the worst case scenario of the obfuscation -- lack of pagecache leads to as many as possible file ops going through obfuscator and being forwarded. 
Otherwise, they could have been absorbed by cache, which leaks strictly no more.
2) conform to our observation on \tz{} -- limited RAM, a luxury to have large enough cache to hold working sets, and it is also the reason why they have to forward file ops in the first place.






\paragraph{Microbenchmarks.}
To understand the overhead of \sys{}'s security mechanisms, we stress \sys{}
with Iozone v3.482~\cite{iozone}, a widely adopted \fs{} benchmark suites for Linux. 
To exclude the benefit of cache and measure the security overhead directly, we set \code{O\_DIRECT} in file APIs to force each read/write to hit \sys{}.


\paragraph{Macrobenchmarks.}
To understand \sys{}'s end-to-end impacts, we run the three IO-intensive benchmarks from well-known test suites. 


\begin{myenumerate}
	\item \textbf{Video}: a sample workload from filebench~\cite{filebench}, representing a continuous surveillance service. 
	It has two sets of videos, one active set that will be actively served and one inactive set that contains outdated videos that will be replaced. 
	It actively reads one video file from the active set, and periodically writes to one file of the inactive set to replace it.
	
	\item \textbf{Web}: 
	a sample workload from filebench~\cite{filebench}, representing a web server deployed on the edge device.
	It serves tens of small files distributed in different directories by continuously opening all of them, reading the whole files, and closing them;
	it logs file operations and appends to a separate log file periodically.  
	
	\item \textbf{SQLite}: 
	SQLite's \code{speedtest} benchmark suite processing queries on a database\cite{sqlite-speedtest}.
	It performs more than 50000 insert, select, update, and delete operations on the table, with varied arguments (e.g., ordered/unordered, indexed/non-indexed).
\end{myenumerate}


We report end-to-end metrics: 
the throughput of \textbf{Video};
the IOPS of \textbf{Web};
the total execution time of \textbf{SQLite}.












==> exp_conf.tex <==



\begin{table}[t!]
\centering
\caption{Experiment Setup}
\label{exp_setup}
\begin{tabular}{|l|l|l|}
\hline
        & \begin{tabular}[c]{@{}l@{}}Value \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Description 
        \end{tabular} \\ \hline
RTT & 64.5ms & WiFi roundtrip time\\ \hline
Up & 0.94Mbps & WiFi uplink bandwidth\\ \hline
Down & 4.12Mbps & WiFi downlink bandwidth\\ \hline %

\end{tabular}
\hspace{-20pt}
\end{table}




==> extras.tex <==
\subsection{Inter-processor coordination}

\paragraph{Execution handoff}
As mentioned above, the main CPU and the PM core run alternately:
for suspend, the kernel powers off the CPU and moves its execution to the PM core;
at the end of resume, the kernel moves its execution back to the main CPU. 

In the execution handoff, we keep the kernel oblivious to the PM core internals. 
Upon moving to the PM core, the kernel passes a snapshot of the CPU state -- containing various register values -- to the \engine{}; 
when the kernel execution leaves the PM core, the \engine{} passes back a snapshot of its \textit{virtual} CPU state. 
This is analogous to virtual-to/from-physical migration in full-fledged virtual machines~\cite{vmware-v2p}; the major difference is that our ``physical'' CPU is much more powerful than the ``host'' -- the PM core.


\paragraph{Interrupt routing}
In suspend/resume, the OS relies on interrupts to learn the power states of IO. 
When handoff happens, the responsibility of interrupt handling must be transferred \textit{atomically}, since one interrupt event can only be handled once. 
To do so, the \engine{} populates the PM core's interrupt vectors according to that of the main CPU;
it then redirects future interrupt events from the main CPU to itself (or vice versa), by reconfiguring the platform interrupt controller.
The main CPU, on the other hand, is kept oblivious.


==> fig-backstore.tex <==
\begin{figure}
\centering
	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/backstore}
	\caption{Backstore and the separated filedata/metadata path. XXX sybil file ops; sybil disk requests; sybil block devices;}
	\label{fig:backstore}
\end{figure}


==> fig-block-access-rule.tex <==
\begin{figure}
\centering
	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/block-access-rule}
	\caption{Block-level access rule of the storage}
	\label{fig:block-access-rule}
\end{figure}


==> fig-block-traces.tex <==
\begin{figure}[h!]
	\vspace{-4mm}
	\centering
	\includegraphics[width=0.4\textwidth{}]{./figs/plot/macrobench/block-traces}
	\vspace{-3mm}
	\caption{Block traces when performing sequential writes to the same file for same size on \code{f2fs} twice, comparing unmodified \code{f2fs} and \code{f2fs} protected by obfuscation surface.
	X-axis: time, Y-axis: block number.}
	\label{fig:block-traces}
	\vspace{-3mm}
\end{figure}


==> fig-btt-ops.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/btt-ops}
	\caption{BTT ops w/ causes XXX:add file access pattern and secrets? --- lwg:obsolete}
	\label{fig:btt}
\end{figure}


==> fig-btt.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/btt}
	\caption{Block translation tables XXX:virt block shall be the same}
	\label{fig:btt}
\end{figure}


==> fig-buddy-binding.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.46\textwidth{}]{./figs/buddy-binding}
	\caption{Buddy file binding procedure, same color means files are in the same buddy group}
	\label{fig:workflow}
\end{figure}


==> fig-cow-comp-ratio.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/cow_comp_ratio}
	\caption{Emu disk size}
	\label{fig:cow-comp-ratio}
\end{figure}


==> fig-disk-heatmap.tex <==
\begin{figure}[h]
	\centering
	\begin{minipage}{0.45\textwidth{}}
		\includegraphics[width=\textwidth{}]{./figs/plot/op_breakdown/plot}
		\caption{Metadata ops breakdown of each benchmark. XXX a table XXX?}
		\label{fig:op-breakdown}
	\end{minipage}
	
	
\end{figure}


==> fig-eg.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.46\textwidth{}]{figs/rw_seq_large}

	~ %
	\vspace{-5pt}		%
	\caption{Workflows of File I/O. We assume that all read()s and write()s are cached. {OBSOLETE}}
	\label{fig:sequence}
	\vspace{-10pt}		%
\end{figure}


==> fig-filebench.tex <==
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=\textwidth{}]{./figs/plot/macro/macro-span}
	\caption{\sys{}'s impact on application performance.
	Upper:\ext{}; lower:\ffs{}.
	X-axis: obfuscation strength \K{};
	On both metadata-intensive and data-intensive benchmarks, \sys{} outperforms alternative designs significantly.
	XXX: logscale may not be a good idea}
	\label{fig:macro}
	\vspace{-1mm}
\end{figure*}


==> fig-history-model.tex <==

\begin{figure}%
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/fig-history-model}
	\caption{	
	FS op model to describe the trustlet behavior
	\textbf{XXX: n-gram, namespace out of date.}		
	}
	\label{fig:history-model}
\end{figure}


==> fig-macrobenchmarks.tex <==
\begin{figure*}
	\begin{minipage}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/macrobench/seq-read}
		        \subcaption{Sequential Read}
		\label{fig:eval:seq-read}
	\end{minipage}
	~
	\begin{minipage}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/macrobench/seq-write}
		\subcaption{Sequential Write}
		\label{fig:eval:seq-write}
	\end{minipage}	
	~
	\begin{minipage}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/macrobench/rand-read}
		        \subcaption{Random Read}
		\label{fig:eval:rand-read}
	\end{minipage}
	~
	\begin{minipage}[b]{0.25\textwidth}
	\includegraphics[width=1\textwidth]{figs/plot/macrobench/rand-write}
	\subcaption{Random Write}
	\label{fig:eval:rand-write}
	\end{minipage}	
	\vspace{-15pt}		%
	\caption{Read/write microbenchmarks with the metadata stencil and operation verifier turned off.
	}

	\label{fig:eval}
\end{figure*}


==> fig-mem.tex <==
\begin{figure}%
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/plot/macro/mem}
	\caption{Memory overhead introduced by \sys{}.}
	\label{fig:mem}
	\vspace*{-1mm}
\end{figure}


==> fig-memoiz.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\textwidth{}]{./figs/plot/macrobench/filebench/cache}
	\vspace{-4mm}
	\caption{Impact of different sizes of secure page cache with and without memoizing validations. File size is 512KB and the network RTT is 50ms. Dashed line shows native (insecure) performance.}
	\label{fig:memoiz}
	\vspace{-4mm}
\end{figure}


==> fig-microbenchmarks-span.tex <==
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=\textwidth{}]{./figs/plot/micro/microbench-span}
	\caption{Microbenchmark performance of \sys{} compared with native, insecure \fs{}s and two alternative designs:K-FS and K-Files.
	\sys{} only incurs up to 31\% throughput drop.
	Upper:\ext{};lower:\ffs{}.
	X-axis: obfuscation strength \K{}.
	}
	\label{fig:micro}
	\vspace{-1mm}
\end{figure*}


==> fig-microbenchmarks.tex <==
\begin{figure}[t!]
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1\textwidth]{figs/plot/ubench/msg-passing}
		        \subcaption{Message Passing}
		\label{fig:eval:msg-passing}
	\end{minipage}
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1\textwidth]{figs/plot/ubench/metadata-stencil}
		        \subcaption{Metadata Stencil}
		\label{fig:eval:metadata-stencil}
	\end{minipage}	
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1\textwidth]{figs/plot/ubench/op-verifier}
		        \subcaption{Operation Verifier}
		\label{fig:eval:op-verifier}
	\end{minipage}	
	\vspace{-5pt}		%
	\caption{A list of microbenchmarks
	}

	\label{fig:eval}
\end{figure}


==> fig-motiv-shuffling.tex <==
\begin{figure}[h]%
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/plot/latency/foo}
	\caption{Strawman designs: shuffling vs sybil data}
	\label{fig:motiv:shuffling}
	\vspace{-0.5em}
\end{figure}


==> fig-mount-sybil.tex <==
\begin{figure}
	\includegraphics[width=0.4\textwidth{}]{./figs/mount_cost}
	\caption{Mounting costs of sybil fses. LWG:may go}
	\label{fig:mount-sybil}
\end{figure}


==> fig-mutual-info.tex <==
\begin{wrapfigure}{r}{0.25\textwidth}
	\includegraphics[width=0.25\textwidth{}]{./figs/plot/mi/plot}
	\caption{Mutual information reduces to negligible with injected delay}
	\label{fig:mi}
	\vspace*{-1em}
\end{wrapfigure}


==> fig-obfuscate.tex <==


\begin{figure}%
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/dtw/dtw}
	\caption{	
		Warping paths of the \textit{real} trace and the \textit{optimal} trace with the observed trace, where the \textit{optimal} trace is calculated by Dynamic Time Warping algorithm over all possible combinations given a set of file system operations and number of the operations. Benchmark: Video.
	}
	\label{fig:dtw}
\end{figure}




==> fig-op-model.tex <==

\begin{figure}%
	\centering
	\missingfigure[figwidth=0.45\textwidth]{fs op transition graph}
	\caption{	
	FS op model to describe the trustlet behavior		
	}
	\label{fig:op-model}
\end{figure}


==> fig-open-latency.tex <==
\begin{figure}[h]%
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/plot/latency/foo}
	\caption{Normalized latency impacts of \sys{} with different \K{} on 9 other file system calls implemented in addition to read/write.
	Upper: \ext{}, lower:\ffs{}}
	\label{fig:latency}
	\vspace{-0.5em}
\end{figure}


==> fig-path-traversal.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.46\textwidth{}]{./figs/plot/macrobench/path-traversal}
	\label{fig:path-traversal}
	\caption{Path traversal latency}
\end{figure}


==> fig-perf-breakdown.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.46\textwidth{}]{figs/plot/macrobench/filebench/perf-breakdown}
	~ %
	\caption{Application latency of the \textbf{Camera} app, showing the comparison among native (insecure), the  execution time with that of adopting \code{UNTRUST} and \code{TRUSTED} api. Network RTT is 100ms.}
	\label{fig:app}
	\vspace{-3mm}		%
\end{figure}


==> fig-real.tex <==
\begin{figure}[ht]%
	\vspace{-0.5mm}
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/plot/latency/breakdown}
	\caption{Execution time breakdown of \sys{} on \code{read} and \code{write} on \code{ext4} (upper) and \code{f2fs} (lower). \textbf{XXXXXX this is normalized. what message does this convey? XXXXXX}}
	\label{fig:breakdown}
	\vspace{-0.5em}
\end{figure}


==> fig-replay.tex <==
\begin{figure}
    \centering
        \vspace{1pt}
        \includegraphics[width=0.4\textwidth{}]{./figs/replay}
        \caption{\sys{} generates sybil traces by replaying historic actual traces, recorded offline and online}
        \label{fig:replay}
   \end{figure}
    

==> fig-sqlite-oram.tex <==
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/sqlite_oram}
	\caption{SQLite Ours vs ORAM}
	\label{fig:sqlite-oram}
\end{figure}


==> fig-strawman.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/strawman}
	\caption{Obfuscation featuring both shuffling and sybil files.XXX:place (1) on the left, pointing only to actual file XXX needed?? XXX The trace library }
	\label{fig:strawman}
\end{figure}


==> fig-toy-eg.tex <==
\begin{figure}[]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/toy-eg}
	\caption{Obfuscation results.
	One obfuscated file trace may map to multiple possible file traces of the trustlet thus increasing the uncertainty of an attacker.
	XXX:can bake this into Figure 4????
	YYY:the key is to show attacker cannot map back to original file trace}
	\label{fig:toy-eg}
\end{figure}


==> fig-workflow.tex <==
\begin{figure}[]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/workflow2}
	\caption{A static view of obfsucated file trace with \sys{}.
\textbf{	XXX: This can stay be need to be updated to reflect trace library, independent timing, etc.}
	}
	\label{fig:workflow}
\end{figure}


==> fig_latency.tex <==

\begin{figure}[t!]
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1.1\textwidth]{figs/plot/read}
		        \subcaption{read}
		\label{fig:eval:read}
	\end{minipage}
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1.1\textwidth]{figs/plot/write}
		        \subcaption{write}
		\label{fig:eval:write}
	\end{minipage}	
	\begin{minipage}[b]{0.15\textwidth}
		\includegraphics[height=1.1\textwidth]{figs/plot/fsync_2}
		        \subcaption{fsync}
		\label{fig:eval:fsync}
	\end{minipage}	

	\caption{A comparison of file I/O latencies
	}
	\vspace{-15pt}		%
	\label{fig:eval}
\end{figure}


==> fsbenchmarks.tex <==

\subsection{title}

==> impl-old.tex <==

\section{Implementation}
\label{sec:impl}



\subsection{The virtual disks}
\note{preserve block semantics}
\sys{} protects the disk hardware in the secure world. 
At the world boundary, it exposes multiple block devices for the normal world OS to operate. 
Actual or sybil, these block devices have the identical interfaces as normal block devices. 
As a result, existing \fs{} implementations and semantics work with \sys{}'s block devices out of box. 

\note{intercept the block reqs}
The difference is that block requests submitted to these block devices will trigger world switch and be interpreted \& executed by \sys{}. 


\note{actual partitionings of system components}
Of the Raspiberry 3 board, we run \sys{} inside the TEE atop OPTEE 4.2
and the untrusted OS with its \fs{} in the normal world. 
By design, the TEE should isolate the physical disk; 
due to OPTEE's lack of disk drivers, our current implementation works around it by isolating the disk in a virtual machine (VM) hypervisor of the same board that is more privileged than the untrusted OS.
To this end, we run the KVM XX.XX and Linux 4.14 as the hypervisor;
the TEE accesses the physical disk by communicating with the hypervisor. 
In summary, our implementation partitions the functions as follows: 
the untrusted OS: a guest OS (Linux 4.14) atop KVM in the normal world; 
the physical disk: in the KVM hypervisor; 
the \sys{} logic: in the TEE. 

\note{normal vs TEE \& interaction}
The hypervisor manages a physical microSD card as the isolated physical disk.
On the physical storage, the hypervisor reserves two regions and exposes them as two block devices dev0 and dev1, each spanning a contiguous range of blocks. 
They serve the actual \fs{} and the syibl images (their metadata blob), respectively. 

\note{tee vs storage interface}
\sys{} passes through disk ops from the actual \fs{} image to dev0; 
the space of dev0 is managed by the \fs{}. 
\sys{} emulates all sybil images on dev1. 
For simplicity, it manages the dev1 space with sequential allocation, whenever a metadata block needs to be materialized/instantiated.
We did not notice any \fs{} slowdown caused by the allocation strategy. 

\subsection{Block translation tables (BTT)}

\input{fig-arch}

\note{Where is BTT? between TEE  and actual storage}
Upon receiving disk ops from \fs{}s, the TEE translates \fs{}-visible disk blocks to the physical blocks with its private Block Translation Tables (BTTs).
A BTT is a per-\fs{} lookup table which maps a logical block of a \fs{} onto a physical block in ether dev0 or dev1. %
It bookkeeps the mappings for all metadata blocks of a \fs{}.
Hence a missed BTT look up indicates an invalid access of metadata (i.e. rogue read), or it is a filedata access;
in either case, \sys{} can safely and silently reject it or drop it as describe in Section~\ref{sec:sybil:paths}

\note{BTT vs FSNR}
With BTTs, the TEE manipulates sybil \fs{} images at low cost. 
To fork a \fs{} image, \sys{} simply duplicates its BTT without duplicating the disk blocks; 
to rename two \fs{} images, \sys{} unmounts the images, exchange both their BTTs, and mounts them back;
to retire a image, \sys{} simply frees its BTT. 

\note{CoW}
For CoW, identical metadata blocks of different \fs{} images are mapped to the same physical block on disk (dev1). 
This is implemented by pointing their BTT entries to the physical disk block.
When the metadata block is written by any of the sharing \fs{}, 
\sys{} allocates a new metadata block for the \fs{}, and updates BTT entries of all sharing images accordingly. 

\paragraph{Store BTTs securely}
A key challenge to BTT is how to store them. 
BTTs should enjoy the same level of confidentiality and reliability as the \fs{}, e.g. with crash consistency. 
How to store BTTs is a chicken-or-egg problem. 
While one may build a filesystem (with crash consistency, redo logging, etc.) inside \tz{} for BTTs, 
doing so is incompatible with our goal of making \tz{} free of \fs{} code. 
Instead, the TEE follows the outsourcing approach and stores \textit{encrypted} BTTs in the normal world, e.g. in sqlite in our implementation. 


\note{BTT security}
The outsourced BTTs leak no secrets: 
BTT lookups are driven by disk ops submitted from the OS; the input block numbers are from the OS; the output block numbers are encrypted.  %
The TEE updates BTTs following the egalitarian principle. 
In renaming \fs{} images, the TEE re-encrypts all their BTT entries so that the OS could not detect the updated BTT entries and hence track the image lineage. 
To allocate a new disk block due to CoW, the TEE re-encrypts all the BTT entries pointing to the shared physical block. 
This is because updating only the BTT entry pointing to the new block will leak image identities. 
Because in response to CoW the TEE always allocates new metadata blocks from the metadata blob (dev1) and assign to sybil images, 
the OS will see that the actual image's BTT entry always retains the same encrypted value. 
This resonates with oblivious access for egalitarian impressions as well~\cite{oram}. 

\paragraph{Other \sys{} metadata.}
Besides BTT (\S~\ref{sec:impl}), in total there are two other data structures need to be persistent: 
\Note{this can go into BTT}
1) for managing emu disk.
This includes a table for tracking the sharing of physical sectors and for bookkeeping sector allocation information.
For a emu disk of 233 MB which can host 19 2GB sybil \fs{}s, the former table consumes only tens of megabytes and the latter consumes tens of bytes.

2) for keeping track of \fs{} lineage (\S~\ref{sec:design:fsnr}), which is bounded by the total number of \fs{}s, usually of tens of bytes.
These data structures need strong crash consistency guarantee as BTT hence are stored unequivocally encrypted using symmetric key \note{XXX} in normal world \fs{}.

In terms of user files, their filenames are encrypted but not filedata because they never go through the OS; 
metadata of any \fs{} are not encrypted because the OS is entitled to owning them.
The key is baked inside the \sys{} binary together with OPTEE OS, hence sealed inside secure world.

\Note{---- below not needed ----}

The metadata store consists of two important metadata, namely BTT and trace library;

\paragraph{Why it's okay to expose metadata store?}
\note{this can serve as a part of security analysis}

\begin{myitemize}
	\item \textbf{BTT} Metadata store supports the four operators of BTT via usual \code{read, write}, whose file traces are listed in Figure~\ref{fig:btt}.
	Following our taxonomy in \S\ref{sec:motiv:case}, the secrets which traces carry are both timing and intra-file access pattern (e.g. one metadata block request leads to one BTT lookup).
	
	However, exposing them does not leak extra information of \sys{}.
	Fundamentally, this is because BTT is incarnated into the \fs{} logic by design -- the timing of each metadata block request and its queried content (i.e. the block number) is driven and already known to the OS!  
	Further, the queried result as of the secure disk sector is encrypted, which leaks no information.
	
	\item \textbf{Storing the trace library} At runtime, metadata store reads the library for replaying sybil traces and writes to it in case new file traces are emerging (\S\ref{sec:design:tracernr}).
	While the library is encrypted, its secrets leaked by the file traces are the timing (e.g. when the backstore needs to read in more sybil traces). 
	
	\sys{} protects it using the same timing protection technique applied to trustlet (\S\ref{sec:design:tracernr}): it instantiates independent timers for injecting sybil traces onto the library, so that the attacker can no longer obtain reliable observation on the file trace. 
	
\end{myitemize}






\subsection{Limitations}

1. relies on KVM. 
Restrained CPU \& RAM would hurt performance. 

2. test harness is colocated with VM (untrusted OS). 
This is due to POSIX support of OPTEE.













==> introduction-liwei.tex <==

\section{Introduction}
\label{sec:intro}






Emerging IoT devices are promise to future edge processing. 
A prominent use of these devices is smart sensors. 
Smart meters measure power consumption thus enabling smart grid\note{cite}; smart temperature and humidity sensors digitalize the environment and can thus help make a better living condition\note{cite}. 
These device have a nature to store data.
In the case of sensors, they'll need to store the capturd data for post analysis; in other scenarios, they'll need to store system configurations, credentials, user information, etc.
However, due to the tight budget, they are usually wimpy and vulnerable.
As a result, attacks against other platforms can easily be launched against these devices which usually carry sensitive data.
To worsen the situation, the connection between the device and the cloud can be intermittent and unstable.
This makes entrusting the data solely to the cloud an unreliable solution.

Therefore, IoT devices demand secure local storage.
And we identify the security requirement as four properties such storage system must gurantee 1) \textbf{freshness}: the system must provide the latest version of data. This elimites swapping attack. 2) \textbf{data integrity}: the data must not be rigged during execution. This eliminates XXX attack. 3) \textbf{data confidentiality}: the data content must not be exposed to any third party. This eliminiates XXX attack. 4) \textbf{non-repudiable I/O}: the data must be stored honestly to its destination. This eliminiates XXX attack.

\note{this paragraph is too fat}
Current approaches targeting different platforms mainly take two routes to the four properties. 
The first approach is targeting local device based on the idea of execution isolation.
The isolated exeuction environment is called Trusted Execution Environment (TEE), which gurantees the integrity and confidentiality of code and data inside.
Open Portable Trusted Execution Environment (OP-TEE) leverages ARM TrustZone to implement TEE.
However, it forwards operations to a handler in normal world to carry out operations.
The second approach is targeting the cloud server based on cryptographic file system (CFS) \note{cite}.
Plutus, SiRiUS and other homogeneous work guanrantee data confidentiality and integrity by encrypting data and metadata.
However, these approaches are not easily applicable in the IoT era.
Major drawbacks include the execeedingly large Trusted Computing Base(TCB) and performance overhead. 
OP-TEE relies on the file system in normal world whose code base is huge, complex and buggy\note{cite remzi FAST13}; 
CFS-like systems suffer from excessive operations on encryption and decryption, which cannot be efficiently handled by IoT devices.
To make things worse, IoT devices have a more critical threat model which invalidates much of the prior TCB such as trusted OS or trusted storage.
Like its counterpart--the cloud, they're designed to be always connected to the Internet;
however, unfortunately, unlike its counterpart, they often receive the poorest software support.
This brings new challenges to IoT security.
On one hand, the threat is not new.
There can be a powerful party of interest which has \textbf{full} control of the device's software stack.
On the other hand, these devices need to securely store their data locally in the sense that the four security requirements must be met.

 
To this end, we propose to reconstruct the IoT file system by combining the best of both worlds. 
We base our design on the insight that, on the local device, the hardware mechanism provides the strongest isolation guanrantee; on the cloud, the software stack enjoys the most timely patch and professional management. 


To describe our design in a nutshell, we propose the secure IoT file system 1) host \textit{secure cache} inside TEE, 2) manage its \textit{replicated metadata} on the cloud and 3) be aware of its \textit{block usage}.
The architecture is shown in Figure~\ref{fig:overview}.

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.47\textwidth{}]{./figs/arch2} 
	\caption{An overview of this work}
	\label{fig:overview}
	\vspace{-10pt}		%
\end{figure}


Our contributions in this work are twofold:
\begin{itemize}
	\item We propose a novel file system design.\note{idea is secure data is stored locally, secure metadata is stored remotely. By storing data using TrustZone, we guanrantee data security; by using the cloud, we gurantee the file system skeleton security.}
	\item We evaluate our design on Linux file system using filebench and iozone benchmarks. The results show our design only incurs \note{XXX} performance overhead and is promising. 
\end{itemize}



==> introduction-lwg.tex <==

\section{Introduction}
\label{sec:intro}


To protect privacy-sensitive apps on mobile and smart devices such as smartphones, surveillance cameras, and cleaning robots\footnote{We refer to them as smart devices in the paper}, 
modern ARM SoCs provide \tz{}, a Trusted 
Execution Environment (TEE). 
Assisted by tools and libraries~\cite{trustshadow,tzslicer}, 
app developers encapsulate their privacy-sensitive code as \textit{\trustlet{}s}. 
\tz{} hence isolates the \trustlet{} execution from the rest of the same platform, including the platform's feature-rich OS, e.g., Linux. 
In this way, \trustlet{}s entrust their data with a lean \tz{} runtime~\cite{optee} rather than 
a commodity OS that is regarded much more vulnerable. 
 

\paragraph{\tz{} needs file service}
\Trustlet{}s need to keep their data persistent. 
For instance, 
a \trustlet{} on surveillance cameras for object detection may store machine learning models, labels of detected objects, or video footage for later model retraining; 
a \trustlet{} on voice assistants for processing voice samples stores processed samples for later retrieval; 
a \trustlet{} on a cleaning robot for constructing floor maps stores the maps for future operations. 
Today's smart devices widely use modern \fs{}s such as ext4~\cite{ext4} and F2FS~\cite{f2fs} and rely on the latter's essential features: journaling~\cite{journaling} for high reliability, flash wear-leveling~\cite{wear-leveling} for strong durability, and numerous optimizations for storage speed and space \Note{cite}. 



For \tz{} to use file services, a commonly adopted practice is outsourcing 
(i.e. a partitioned storage stack design \Note{better not call it this way}): 
\note{todo: provide more evidence}
leaving \fs{}s in the untrusted OS
and forwarding file requests (e.g., open/read/write/close) from \tz{} to the \fs{}s \Note{cite}, as shown in Figure~\ref{fig:overview}(a). 
Assuming an honest but curious OS, the \tee{} encrypts file data at the \tz{} boundary. 

The reasons for \textit{not} incorporating filesystems in \tz{} are both security and practicability.
Feature-rich \fs{}s often have sophisticated internals 
(35K SLoC for ext3/4, 17K for f2fs \Note{and for VFS? better nums});
they depend on a commodity kernel, e.g., Linux,  through an in-kernel, brittle binary interface~\cite{transkernel}. 
Pulling these \fs{}s to \tz{} 
adds to the \tz{} both the \fs{} code as well as the extensive kernel services (e.g. memory allocator \Note{better? VFS? block schedulers?}) 
the \fs{} depends on. 
This results in bloated \tz{} TCB (e.g. a typical \tz{} runtime only has XXX SLoC) and hence weakened 
security guarantee~\cite{fs_evo,kernel_bug} \Note{should say fses are often buggy and crashy -- bad for TZ}. 
Doing so would also require maintaining multiple \fs{} versions for disparate runtime environments -- the kernel and for the \tz{}, making maintaining the \fs{} code tedious. 


\input{fig-overview}

\paragraph{Problem: lack of file trace confidentiality}
While requesting external file service has been a popular design, 
the approach exposes file trace to the OS. 
A file trace is a sequence of file operations (\textit{file ops} in short), including operation types (e.g., read/write), accessed file paths, and accessed file offsets, as exemplified in Listing~\ref{code:syscall}.
It has been shown that by observing file traces not the actual filedata, 
a curious OS may infer secrets of \trustlet{}s~\cite{obliviate}. 
\Note{ack this as a know problem; but even the fact of access may leak info -- bad}

\paragraph{Challenge \& contributions}
This paper answers the following question: 
\textit{in requesting external \fs{} services, can \tz{} hide its file trace even from the service provider itself (i.e. an honest but curious OS)?}
To protect access trace privacy, a known approach and also an old wisdom is \textbf{noise injection}\note{cite}: 
the service requester (\tz{} in our case) injects sybil ops as noise into the total access trace; 
by executing the trace, the service provider (OS in our case) fulfills the requester's intent 
while remaining uncertain about the actual trace. 

\Note{paragraphs above and below: good. can be better integrated}

Under the noise-injection approach, the first and foremost goal we seek to achieve is \textbf{transparency} -- injected sybil file ops (i.e. noise) must be transparent to user \fs{}.
This is because \fs{}s are engineered for structured, named data;
their performance and efficiency critically depend on the data layout and their namespace organization. 
We seek to keep the \fs{} image unaffected in the face of noise, so that the \fs{} operates with all its optimizations as effective as if there is no sybil file ops. 

\Note{Can be compressed. A bit slow because the exciting parts are in ``contributions''}

\paragraph{Approach foundation: Multiple sybil filesystems} 
Our foundational approach is a multiple sybil \fs{}s design  -- 
\sys{} instantiates multiple sybil \fs{} instances (alongside the actual \fs{}) with the OS as shown in Figure~\ref{fig:overview}(b).
The sybil \fs{}s serve as the target for \sys{} to inject sybil file ops (i.e. replayed file trace) for hiding the actual file ops while the actual \fs{} is kept transparent.

\Note{forecast: storage is in TZ; covert discard, which seems natural to mention here}


Atop the multiple sybil \fs{} design, \fs{}s, as persistent data stores, pose the following challenges: 
\paragraph{Challenge I: Injecting credible sybil file ops}
\Fs{} is a structured namespace, whose file ops have rich-semantics. 
Injecting random file ops (i.e. white noise) to sybil filesystems will be easily recognized by the attacker (e.g. read from a neg offset). 
The injected sybil file ops must be deceptive, that is, from an attacker's perspective, they resemble a credible trustlet behavior.

\paragraph{Contribution: Egalitarian trace injection} 
\sys{} inject sybil ops by recording file ops from the trustlet and replaying them on sybil \fs{}s.
\sys{} records not only the access pattern of the file ops but also their timings. This results an egalitarian view of file traces, actual or sybil, to all filesystems;
hence the actual file trace blends in sybil file traces and is protected. 


\paragraph{Challenge III: Ensuring low storage overhead}
Without optimizations, large number of sybil \fs{} instances and continuous forking (i.e. described above) incur great storage overhead.
This conflicts with constrained storage on smart devices: slow speed (XXX MB/sec) with limited capacity (tens of GBs). 
To be practical, the resultant disk space cost and access shall scale slowly with the strength of the obfuscation. 

\paragraph{Contribution: Secure backstore} \Note{covert disk emulation?}
\sys{}'s key insight is to have the secure backstore only store sybil \fs{}s' metadata, which is highly similar.
To this end, the secure backstore emulates virtual disks using a Block Translation Table (BTT), which translates a sybil filesystems block number into a compact emulated disk block number.
It implements \textit{covert discard} to silently drop the data read/write block requests to sybil filesystems;
for metadata block requests, secure backstore executes them in a Copy-on-Write fashion to avoid redundancy.
It also emulates the timings for block requests of virtual disks such that they appear indistinguishable from an actual disk that stores the actual \fs{}.


\paragraph{Challenge II: Coping with actual filesystem identity exposure}
Despite the egalitarian view of file traces, long-term observation across the history of them is risky -- once the identity of actual \fs{} is exposed via unexpected channels, its full history can be recovered.
Hence, the attacker's observations must be bound to a limited time window.

\paragraph{Contribution: Continuous backstore namespace randomization} 
\sys{} mounts sybil and actual filesystems on \textit{virtual disks}; 
it implements three operators on the virtual disks: rename, fork, and retiring.
With the operators, the system continuously randomizes the layout of filesystems on virtual disks by shuffling existing filesystems between virtual disks and instantiating new ones from replicating existing ones.
As a result, the attacker's observation is only valid between short randomization round, even when she reveals the identity of an actual \fs{}.


\paragraph{Challenge IV: Own metadata persistence without a filesystem}
The system metadata, most notably BTT, also needs persistence and crash consistency but it needs not to be an in-situ \fs{}. 
Otherwise, user files can be directly stored in the secure world \fs{}, which contradicts our goal -- not inventing nor porting \fs{}s in secure world. 

\paragraph{Contribution: External BTT}
\sys{} outsourced BTT storage to normal world \fs{} like user files. 
Unlike user file access pattern and timing that are protected by egalitarian trace injection, those of the table are visible to OS and synchronous with metadata block requests of all \fs{}s, leaking no extra information.
Hence by storing the BTT externally, \sys{} metadata enjoys a free ride with feature-rich normal world filesystem.









\Note{the following could go to abs}
To summarize, \sys{} is a lightweight \tee{} module and a holistic storage stack solution to trustlet file trace confidentiality. 
\sys{} builds atop a partitioned storage stack spanning the normal/secure worlds.
It keeps the block layer and the underlying disk within the \tz{} (i.e. the secure backstore as in Figure~\ref{fig:overview}) while leaving the \fs{} logic in the OS of the normal world.
It instantiates multiple sybil filesystems and injects egalitarian file traces on them for hiding the actual one;
it keep bare minimum metadata for sybil filesystems to function while keeping the OS oblivious;
it outsources its metadata to normal world filesystem for persistence and crash consistency.

We show \sys{} works with a variety of \textit{unmodified}, modern, and sophisticated \fs{}s, e.g., ext3/4 and F2FS. 
We demonstrate the infeasiblility of recovering the actual file trace after obfuscation. 
We show that such \K{}-anonymity hence mitigates known attacks via side channels of file trace.
We demonstrate that with \sys{}'s optimizations, the seemingly aggressive and expensive obfuscation only incurs moderate overhead even on intensive \fs{} benchmarks, e.g., \note{XXX}\% slowdown and \note{YYY}\% additional storage space with $K$ as high as 20. 

This paper makes the following contributions:
\begin{myitemize}
\item We demonstrate attacks against \tz{}'s current \fs{} services, showing that file trace can be exploited as a side channel in order to break \tz{}'s data confidentiality.
\note{we formalize the attack} into a framework...

\item We present \sys{} for protecting file trace confidentiality. 
\st{Applying \K{}-anonymity}, \sys{} comes with novel designs of \multifs{}s and decoupled storage layer.
By design, \sys{} works with many mature/modern \fs{}s with no modifications. 

\item We conduct security analysis of \sys{}, showing that it effectively mitigates the file trace side-channel attacks.

\item We build and evaluate \sys{}, showing minor overhead (31\%) even with a large \K{} (20) and under intensive \fs{} benchmarks. 

\end{myitemize}





==> limitation.tex <==



==> macro-apps.tex <==

Real-world applications



==> macrobenchmarks-bak.tex <==

\input{fig-filebench}
\subsection{Macrobenchmarks}
\label{sec:macrobenchmark}

We answer the following questions:

\Note{fig 5/6 may use linear scale}

\begin{myenumerate}
	\item What are the end-to-end execution overheads of \sys{}? How do such overheads escalate as \K{} increases?
	\item How do \multifs{}s mitigate the overhead?
	\item What are the storage/memory overheads of \multifs{}? 
\end{myenumerate}


\paragraph{\note{30\% sounds impossible, why?}}

1. The multiple orders of magnitude latency diff between IO device and fs~\cite{relaytracer} (cite more).
In this platform, our experience is IO is 50x slower than fs.
A larger difference is foreseeable as smart devices get beefier CPU.

2. \fs{}s are scalable and parallel~\cite{fs-scalability} in this 8-core platform. 
There is little data dependency between the \fs{}s and files.

3. We are counting trustlet throughput, whose counting ends at the last actual file op.

\paragraph{Throughput loss.}
As shown in Figure~\ref{fig:macro} (a), \sys{} is insensitive to the increase in \K{} and incurs a negligible throughput loss (up to 1.2\% when \K{} = 20 on \ffs{}) for the \textbf{Video} benchmark on both \fs{}s, because for the continuous \code{read} operations, \sys{} only does actual disk IO for real ops but not the sybil ones and that the \code{write} is periodic (i.e., per 10 seconds), which further amortizes the throughput loss.

For \textbf{Web}, \sys{} incurs more noticeable throughput loss, shown in Figure~\ref{fig:macro} (b).
As \K{} increases from 5 to 20, the IOPS drops by 49\% (on \ffs{}) to 59\% (on \ext{}).
This is due to the benchmark is metadata-intensive: when \K{} = 20 and 50 user files are being actively worked on, the total number of files seen by the normal world OS reaches 1000, which generates large traffic of metadata block requests.

\paragraph{Prolonged execution time.}
Compared with \textbf{Video} and \textbf{Web} benchmarks, \textbf{SQLite} has a mixture of data-intensive and metadata-intensive workloads,
our results show \sys{} adds moderate overhead to the \textbf{SQLite} benchmark.
As shown in Figure~\ref{fig:macro} (c), \sys{} extends the overall execution time by up to 46\% (\K{} = 20 on \ffs{}).

\paragraph{Comparison with alternative designs.}
On both metadata-intensive and data-intensive benchmarks, \sys{} outperforms alternative designs significantly: \textbf{K-FS}'s performance is upto 102$\times$ worse while \textbf{K-Files}'s performance is up to 1.5$\times$ worse (in \textbf{Web}, \textbf{K-Files} populates the \fs{}).


\paragraph{Overhead impacted by \fs{} design.}
For data intensive workloads (i.e., \textbf{Video} and \textbf{SQLite}), \sys{} incurs 38\% higher overhead in \ffs{} than in \ext{}. 
This is because when the working sets are relatively small (i.e., tens of files), the more sophisticated execution logic generates contributes more to the overhead.
For example, in the same benchmarks, we saw sometimes 10$\times$ more block requests are generated by sybil \ffs{} than \ext{}.
We quantitatively show the breakdown of execution time in both \fs{}s in \S~\ref{sec:microbenchmark}.
Interestingly, for metadata intensive workloads (i.e., \textbf{Web}), \sys{} on \ffs{} outperforms \ext{}, likely due to \ffs{}'s different internal structure: it groups a set of most often used data blocks, and thus has better locality than \ext{}.



\Note{todo: showing plots for comparing storage/mem overhead vs alternatives}

\paragraph{Storage overhead}
Possessing only metadata blobs for \multifs{}s, \sys{} is space-efficient.
A 4GB \ffs{} and \ext{} \multifs{} only requires 13MB and 130MB of physical disk blocks to store metadata blobs in the secure backstore, which accounts for 0.3\% and 3\% storage overhead respectively.
In comparison, for each 4GB \multifs{}, both \textbf{K-FS} and \textbf{K-files} lead to \K{} - 1 times storage space waste.
\textbf{K-FS} requires full physical disk space for each \multifs{}; 
\textbf{K-Files} can only achieve a storage overhead on par with \sys{} if it only works on a file strictly smaller than 665KB in a \ffs{} or 6.5MB in a \ext{} \fs{}, which is hardly realistic and applicable.



\paragraph{Memory overhead.}
\input{fig-mem}
We compare the system memory usage when benchmarks are run without \sys{} and with \sys{} (\K{} = 20).
\sys{} increases the memory overhead by less than 8\% even when \K{} = 20, because the commodity OS caches the metadata of \multifs{}s (as it sees no difference).




\paragraph{Comparisons with ORAM}
ORAM causes orders of magnitude slowdown



==> methodology-old.tex <==

\section{Design Sketch}

Given that suspend/resume procedure is time-consuming and IO bound, our key insight is that its efficiency can benefit from extremely asymmetric CPU cores. 
\paragraph{Architectural assumption}
Power domain, wakeup source, shared memory, different ISA, ....
Conceptually, such a weak core is capable of performing suspend/resume on behalf of the strong cores.
In particular, we seek to minimizing the on time of strong cores by offloading the execution of suspend/resume to a weak core. 

This seemingly simple goal raises a great deal of challenges, in particular from kernel complexity. 
First, as discussed in Section XXX, the OS code for suspend/resume is complex and invokes a variety of other kernel subsystems.
Second, the hardware discrepancy -- from ISA to memory model -- between asymmetric cores can be huge. 
Third, 

\paragraph{Reflection on K2}
In our prior work K2~\cite{k2} we explored the design of spanning one OS image over highly asymmetric processors. 
As a generic approach for OS refactoring, OS argues for ....
One major drawback of this approach, as we found out in practice, is that it tightly couples the kernel instances (software stack instances) running on different processors. 
This entails two requirements: 
first, the kernel images (as their respective native binaries) must be generated from one unified kernel tree, and every memory object must be placed at the same virtual address;
second, the weak core must run a full-fledged Linux (VM enabled). 
The resultant efforts are substantial (and repetitive) across Linux kernels of different versions or for different SoCs: 
it requires porting kernel trees (e.g. for x86 or ARMv7) to the weak core (which, due to its embedded profile, often receives poor or no support from the mainline kernel) and manual tweaking of kernel configurations, linker commands, and the internal memory layout of data structures.

However, treating a specific, IO-bound kernel procedure (suspend/resume) allows us to explore a design point that is other than K2: 
we trade the kernel execution overhead of the weak core for minimizing coupling and efforts craft the kernel \textit{per se.}.
Thus, we take an extreme design point -- using the weak core as a (software-accelerated) virtualization engine for host kernel execution -- only the suspend/resume path.
This new perspective enables us to retrofit rich results in virtualization.

The top challenge, however, is execution efficiency: 
the weak core has to execute binary in a different ISA;
this, combined with its lack of hardware features (e.g. no MMU or virtualization hardware), may lead to 

\Paragraph{Programming challenge}

This has to be done in software. registers have to be saved and restored. drivers have to decide the PM policies and the order of suspending.

the little PM core -- for efficiency, can be very wimpy. We simply do not assume it has virtual memory hardware. It, however, has access to the DRAM.

(can it access the main DDR? shall we design under memory constraints? this may enable sensor hubs with limited local memory, making our work more generic)


Heterogeneity -- the PM core and the main CPU may differ on ISAs (even ARM cores start to move to 64 bits)
Simply cannot ask for homogeneity.

\Paragraph{Interrupt handling}



==> microbenchmarks-bak.tex <==
\input{fig-microbenchmarks-span}
\input{fig-open-latency}
\subsection{Microbenchmarks}
\label{sec:microbenchmark}

We run the aforementioned stress test to understand the overhead of \sys{}'s sybil file and \fs{}s.



\paragraph{Throughput impacts.}
\sys{} maintains an affordable overhead and is resistant to the increase of \K{}.
As \K{} increases by 4$\times$ (i.e., from \K{} = 5 to \K{} = 20), the overhead only increases by up to 31\% (\ffs{}, sequential read).
When \K{} is large (i.e., 20), it only incurs an average of 20\% throughput drop, compared with the native \fs{}.
In comparison, \textbf{K-FS} which executes block IO for each \K{} file is at least 19$\times$ slower than the native version and its throughput further degrades linearly with $\K{}^2$, considering \K{} ops will be applied to \K{} files.
As expected, \textbf{K-Files} has a very similar performance with \sys{}, due to block requests of sybil ops are dropped.




\paragraph{Latency impacts.}
We show \sys{}'s impacts on 9 file system calls in Figure~\ref{fig:latency}.
As expected, meta ops (\code{ftruncate}, \code{fchmod}, \code{fchown}, \code{mkdir}, and \code{unlinkat}) that will change metadata, their latency increases linearly with \K{} (up to 17$\times$ when \K{} = 20 on \ext{}).
This is because all \multifs{}s have to carry out these ops and do the actual block IO, causing \K{} times more block traffic.
In comparison, ops such as \code{fsync} and \code{close} do not suffer as much, with 2.4$\times$ and 7.9$\times$ overhead respectively. 
This is because they only need to carry out the block IO requests for the real user file but not \files{}.







\noindent
\textbf{Cross-world invocations.} 
It only takes few thousand nanoseconds for the normal world \fs{} to receive file APIs sent by the TEE, and vice versa. 
Within a cross-world invocation, the world switch takes around 49ns, accounting for less than 1\% time for all benchmarks.

\paragraph{Storage model overhead}















==> microbenchmarks.tex <==


\subsection{FSNR overhead}
\input{fig-mount-sybil}

\input{fig-fsnr-perf}

Show: file access delays as the FSNR interval changes. 

Breakdown: 
\begin{myenumerate}
	\item 
	mounting costs of sybil fses...
	
	\item 
	costs to run fsnr, that is, costs of forking, renaming, \& retiring. 		
\end{myenumerate}


\paragraph{Performance impacts of different fsnr interval.}
Figure~\ref{fig:fsnr-perf} shows how trustlet-perceived delay changes with fsnr intervals, in a 20-fs setup.
Since CredentialManager involves only one round of whole file read, it does not go through FSNR and we omit its results discussion below.
On a 1s-interval of FSNR, \sys{} increases the delay by 6$\times$ - 29$\times$ (on average 19$\times$) than baseline (i.e. w/o any protection), with an average of 40 FSNR per benchmark.
As FSNR frequency becomes more aggressive, e.g. at a 100ms interval, the delay quickly escalates to 45$\times$ - 273$\times$ than baseline.
Despite this, \sys{} still performs much better than strawman: 
at a 1s-interval, \sys{} has an average of 36$\times$ smaller delay; 
even at 100ms-interval, it is still on average 7$\times$ faster.

The major reason causing the overhead is that FSNR is very sensitive to (large) number of \fs{}s;
we breakdown their costs and show in Figure~\ref{fig:mount-sybil}.
There are two factors for such sensitivity: 
1) mounting costs are non-negligible. 
On average, mounting a \fs{} on Rpi costs around 80ms, actual or sybil. 
This is very costly, accounting even for a large portion of the benchmark execution time (e.g. 20\% for SQLite, 34\% for Lucy).
We suspect this is because unlike the read/write paths of \fs{} code, the mount path is less optimized.
2) current FSNR is sequential.
During each round of FSNR, \sys{} sequentially unmount individual \fs{}s, renames/forks them, and mount them back, each costing around 100ms.
As a result, the delay quickly escalates, linear to the number of \fs{}s.  

The results suggest interesting tradeoffs between the frequency of FSNR and the delay it causes.
On one hand, depending on the trustlet's workload and its native execution time, one must judiciously select an interval such that FSNR does not dominate the delay.
On the other hand, further optimizations can be done to accelerate and enable more frequent FSNR.
Finally, we'd like to stress FSNR can be done in an offline manner, which does not increase trustlet-perceived delay, e.g. as in CredentialManager. 

\paragraph{FSNR atomic ops}
Figure~\ref{fig:mount-sybil} shows the overhead of three atomic operations of FSNR:
\begin{myitemize}
	\item \textbf{Forking}. 
	The most expensive op across all due to memcpy. 
	It is strictly linear to the BTT size: 
	\note{TODO:update}
	Smallest size (e.g. 128MB) takes ~100ms while 2GB takes 800ms
	
	\item \textbf{Renaming}. 
	The costs are minor, linear to BTT size and come from data encryption.
	We measure it using AES encryption scheme with NEON instructions enabled -- 
	for a 64MB sybil \fs{} it takes 16ms and for a 2GB sybil \fs{} used in Lucy, it takes 510ms. 
	
	\item \textbf{Retiring}. 
	It incurs minimal costs and costs less than 1ms because it simply drops BTT \& decrement ref count inside \tee{}.
\end{myitemize}

The above minor overheads to adding, deleting, and shuffling \fs{}s at ease are enabled by BTTs, which replace expensive physical disk ops with cheap memory ops;
What is more, the costs only grow linearly with \textit{metadata} size but not the \textit{whole disk} size.









==> motiv-bak.tex <==
\section{The problem of forwarding \fs{} calls} 
\label{sec:motiv:observation}

\input{threat-model}





\subsection{Attack vector taxonomy}
\label{sec:motiv:case}


Despite the encrypted file data, trustlets must send file ops and their arguments in cleartext to the OS for execution. 
The OS is able to observe: 
\begin{myitemize}
	\item The types of file ops, e.g. read/write/fstat;
	\item The op arguments, e.g. read/write sizes, offsets, and flags;
	\item The accessed file paths. Note that simply encrypting directory names cannot protect the relative location of an accessed file in a directory tree. 
\end{myitemize}

The sequence of ops observed by the OS constitutes a \textit{file trace}. 
As already shown in prior work~\cite{obliviate,controlledChannel}, a file trace may leak the secrets of its requester (in our case, a trustlet). 


\paragraph{Three attack vectors}
With the above observations on file traces of typical trustlet, we summarize the following three general attack vectors (on access patterns) for exploiting file trace side-channel attack on smart devices: 
\note{todo: finalize the terms}
\begin{myitemize}
	\item \textbf{Timing/occurrence pattern}: the trustlet accesses a single file, whose file trace is trivial (e.g. seq read to whole file, seq append) and does not carry secrets. 
	Rather, its occurrence and timing is the secret which directly correlates to the event (e.g. user authentication). 
	
	\item \textbf{Inter-file pattern}: the trustlet accesses a set of files with trivial file trace. 
	The pattern of which file in the set is being accessed carries the secret (e.g. SSH credential).
	\Note{I wouldn't call it patterns. It's just file paths being accessed.}
	
	\item \textbf{Intra-file pattern (timing)}: the trustlet accesses a single file, whose file trace is non-trivial and secret-dependent (e.g. user queries).
	
\end{myitemize}

These attack vectors are not uncommon on \device{}, as we will next present a trustlet case study for \device{}s to understand their file traces and associated secrets.





\input{tab-app-cases}
\paragraph{App case study}
We study the following typical trustlet examples and how they may be subject to the attacks above. 
\note{can we do reverse mapping on this? focus on types of secrets, etc.}

\begin{itemize}
\item  \textbf{Biometric service}: such as automatic fingerprint identification system (AFIS)\note{cite}. 
Upon matching request, the TA loads a set of fingerprints from disk and builds an in-memory index. 

\textbf{File trace}: whole file seq read.

\textbf{Scenario}: 
The fact of file access reveals (at longer time scale) the usage of the biometric service and therefore user activities. 
For instance, at a certain geolocation (which is known to the OS), the OS observes a TA using fingerprint reader and therefore infers that a financial transaction has happened (\textbf{this may be a weak example}).
 
\item \textbf{Video surveillance} with object detection. 
The TA detects objects of interest (e.g. humans) on video stream. 
Upon detection, it appends video frames to a file. 

\textbf{File trace:} seq append.

\textbf{Scenario:} 
The fact of file append indicates the appearance of humans which are learnt by the attacker. 	

\item \textbf{System log} (or data historian?). 
The TA appends messages to a file. 
The amount of data written and offsets correlate to message types. 

\textbf{File trace:} seq append w/ patterned offset/size. 

\textbf{Scenario:} syslogd? 

\item \textbf{Access credentials.} 
The TA will load key files for validation. 

\textbf{File trace:} access directed to different files.

\textbf{Scenario:} Which file is accessed leaks to which users try to authenticate, e.g. in a SSH server scenario.


\item \textbf{Queries} over Sqlite and ROSbag. 
The TA seeks and reads specifics pages from a big files. 

\textbf{File trace:} data-dependent access pattern. 

\textbf{Scenario:} the attacker who knows file schemas can infer query semantics/parameters and query outcome. 

\item \textbf{Fulltext search and anayltics}. 
The TA takes query, parses index, locates and reads the target file for ML. 

\textbf{File trace:} data-dependent access pattern and file. 

\textbf{Scenario:} The attacker who knows file schemas and file identities can infer query semantics/parameters and hit file targets.

\end{itemize}





We next show why existing techniques are inadequate.



























\subsection{Why disrupting the actual fs image undesirable? -- existing approaches do not work}
\label{sec:motiv:constraint}

\note{goal of this section is to advocate for multi-fs, need motivate record n replay design?}


\begin{myitemize}
\item obfuscation (shuffling) within the actual fs ...
does not address all the attack vectors. 
The problem: disturbing disk layout; performance loss. 

\item sybil ops within the actual fs ...

\end{myitemize}

(can be brief on both -- combine the discussion) 


Towards hiding file traces (activities), there are two existing approaches do it (manipulate, operate on) within one \fs{} -- the actual \fs{} image. 

\textbf{Obfuscation}: ~\cite{obfuscation-book}
As shown in Figure~\ref{fig:strawman}-(1), 
in creating filedata, 
\fs{} clients (trustlets in our case) shuffle (arrange) filedata (blocks~\cite{obliviate} or files~\cite{crocus}) on disk, and keeps the shuffling scheme only known to the clients; 
\Note{be brief:}
the clients send the OS file ops that point to shuffled blocks or files, preventing the OS (\fs{} logic) from learning the access offsets within a file or the accessed file paths (or obfuscating the file access pattern in the view of the OS). 

\textbf{Sybil ops}:
\fs{} clients may inject sybil data (to the actual \fs{} image) and emitting sybil ops that operating on the sybil data, as a camouflage over the actual file ops. 
This is a known approach to data privacy ~\cite{kanon,sybilquery,kloakdb} 
This is shown in Figure~\ref{fig:strawman}(2).
Unable to distinguish the sybil data from the actual data, the OS executes all the ops. 
\note{a more important question is how to generate sybil ops? then we can focus on the performance loss, etc.}


\paragraph{Summary: need for transparency}
The key drawback of only having one \fs{} image -- the actual one -- is that the high disturbance to the \fs{} image as a side effect, which is detrimental to \fs{} performance and efficiency. 
It is difficult to isolate the overhead of strong camouflage from the performance/efficiency of actual file ops. 

For filedata
Shuffling (obfuscation) shatters the disk block address space and \fs{} name space. 
The disk blocks that the \fs{} code sees as contiguous are physically scattered on disk; 
the files that the \fs{} code sees as co-located in the same directory actually come from unrelated paths. 
This breaks crucial performance/space optimizations in \fs{} code that exploit locality in disk layout and directory structures. 
\Note{add}
Figure XXX shows the performance degradation under typical SQLite workload~\cite{sqlite-speedtest} led by the approach.
In the benchmark, the trustlet issues a mix of text, fp, numerics and range queries on a SQLite DB. %
Compared with the original data block layout, shuffling disk blocks within each files reduces the benchmark throughput by up to 76\% (i.e. Range select, TEXT). 
The reason is that applying data shuffling to \fs{}s breaks data locality, a primary goal of \fs{} design,  
turning carefully orchestrated sequential access into random access.

\Note{criticism: what about ``partial shuffling''? is it as bad?}

\textbf{Sybil ops:}
\textbf{what's the relation to shuffling? complementary}
To be deceptive, sybil ops and data shall overshadow the actual one in volume. \Note{evidence?}
As a result, the resultant disk ops and wasted disk space could be orders of magnitude higher compared to the actual data, taxing the storage resource heavily. 
Residing in the same \fs{} image, the excessive sybil data further fragment the actual data, break its locality, slows down the access. 
The net effect is equivalent to the well-known effect of filesystem ``aging''. 
Essentially, excessive sybil data makes the actual \fs{} image \textit{age} much faster, which in turn demand higher management overhead, a symptom well recognized and studied. 
Figure XXX shows a microbenchmark of a full text search. 
The microbenchmark searches and reports any matching strings in a text database consisting of over one thousand files. 
By adding sybil data, the text database is heavily fragmented, causing its performance to drop by $3\times$ on \ext{}. 



\input{fig-strawman}





















\paragraph{Summary -- the need for multiple \fs{}s}
The key to avoid heavy performance penalty is to minimize the impact on the actual \fs{} image. 

To this end, we advocate for instantiating additional sybil \fs{} images as the targets of obfuscation/sybil ops. 
As a result, the actual \fs{} has the exactly same data content and layout as if there is no obfuscation.
All the performance and space optimizations hence work as intended.
The \fs{} boundary becomes the boundary of actual/sybil data and therefore the boundary for (strong?) performance isolation around the actual \fs{} image.  






==> new.tex <==
\paragraph{A Minimal Example}
\note{the following may be useful. but need revision and compression}
To illustrate our initial design, we next describe a file API sequence, in which a client first open()s a file, read()s and write()s to it, and invokes fsync() to make the changes persistent. 

The interaction sequence of our system is shown in Figure \ref{fig:sequence}.
These syscalls invoke file system functions to read required block and saturate memory pages with the data.
First, open() is issued by a secure application out to the file system in normal world. 
Open() gathers the metadata (i.e., inode) of the file and sets up a descriptor for the file to be operated on by iteratively querying the super blocks.
Then, the normal file system walks each (sub)directory along the file path by reading metadata and directory file blocks from TEE to do name comparison 
until it finally reaches the metadata block representing the file we want to open and reads it into memory.
As has been described, our system will pass all the queried super blocks directly out to the file system in normal world as they are metadata.
After getting the in-memory inode of the opened file, the physical location of the file on disks is also known and the file's address space is associated with its entry (i.e. file descriptor) in the file table.
When the secure app wants to read() the opened file, our system will first search among the secure page cache.
A cache hit will return the file data directly to the app.
In case of a cache miss, our system issues read() out to the normal world and sends the same request to the cloud simultaneously.
Then it will examine all incoming block read requests from normal world and validate them with the cloud.
If the validation succeeds (i.e., matching that with the cloud), those blocks are read to fill page cache and returned to the secure app.
Otherwise, the read() will fail. 
mmap() associates the address space of the process with the inode.
It will locate (if necessary, allocate) page cache for this file then setup the entries of the process's page table to corresponding pages.
User can then read/write the file the same way as they do to a memory region.
Similar to read(), when the secure app write() data to the file, our system will first search among secure page cache. 
A cache hit will make our system write data only to the corresponding page cache. 
Otherwise, our system will forward the write() to normal world so that it can allocate blocks for the write().
Subsequently, our system examines and validates all the incoming block write requests with the cloud.

When changes need to become persistent, the secure app invokes fsync() to flush all dirty pages into the storage.
It scans through all dirty pages of the file and issues block write request accordingly.
These block write requests will be forwarded altogether to the cloud for validation.
A successful return on fsync() indicates that up to this point, each read/write is validated to be trusted.


==> obfuscator-amplification.tex <==
\subsection{Amplification rules}

\Note{need some high-level objectives?}

\begin{myitemize}
\item against segmenting attack...?
\item hide the identity of the actual fs... homogenize the views... against differential analysis...
\end{myitemize}


 



To this end, the obfuscator enforces a set of obfuscation rules to administrate the per-op amplification process, as will be detailed below.

\paragraph{Obfuscation workflow}
\Note{useful but too detailed... to revise}

At run time, as a trustlet emits \textit{each} actual file op, 
\sys{} invokes the obfuscator and emits corresponding ops. 
By amplifying per op rather than a sequence of multiple \sys{} avoids introducing buffer delays to file op processing. 

\sys{} amplifies an actual op $X$ in the following procedure: 

\begin{myitemize}

	\item 
	get a random number N=random(1..K-1); 
	invoke the generator get() to generate N sybil ops as a sequence. 
	Insert the actual op X in a random position of the sequence. Get S.
	
	\item 
	\textbf{To actual fs:} 	
	Emit S to the actual fs. 


	\item 
	\textbf{To sybil fses:} 
	
	\begin{myitemize}
	\item 
	If X is a transparent op: Emit S to the all other sybil fses. 	
	
	\item X is non transparent op: 
	for each of the K-1 sybil fs: invoke the generator to get a non-transparent op X. 
	replace the non-transparent op in S while keep others unchanged; emit S to the sybil fs. 
	\end{myitemize}	
		
\end{myitemize}	

Figure~\ref{fig:workflow} shows each step and the overall obfuscated trace.



\paragraph{Benefits}
There are several noteworthy aspects. 
From the view of $K$ traces targeting $K$ \fs{}s, ...

First, the attacker is unable to cluster the output ops corresponding to each input op. 
(She cannot precisely pinpoint a sequence of adjacent ops resulted from the same input op). 
This is because N is non deterministic. 
In particular, even when X is non-transparent op we emits a varying number of transparent op, making the total number non deterministic. 
Then, the obfuscation throttle the flow of the ops...
As a corollary, the attacker cannot determine the number of actual ops. 

unable to do differential analysis over K \fs{}s. 




\subsubsection{Hiding the number of vertical amplifications}
The obfuscator injects transparent sybil ops to the actual file op stream destining to the actual \fs{} to fullfil vertical amplification.


\paragraph{Challenge}
\note{looks a little bit over stretched here}
While serving as the last line of defense, vertical amplification also introduces a new challenge: how to hide the number of vertical amplifications from the OS?
The number is crucial, with which the attacker is much more certain about the actual file trace, as it also determines the total executed actual ops definitely.
\Note{talk about segmenting the observed trace, etc...}




\paragraph{Rule IV. Blur the amplification boundary}
The solution is simple: increase attacker's uncertainty on how many file ops will be injected per amplification.
Hence, for each vertical amplification the obfuscator injects \textit{various} number (e.g. from $1$ to $K$) of file ops. %
Doing so prevents an attacker from inferring a fixed mapping between the number of actual ops and the observed file ops.
For instance, while a fixed mapping allows the attacker to assert \textit{exactly one} file op among a series of $K$ ops is actual, the blurred amplification boundary decreases her certainty -- she only assert \textit{at least one} file op is actual. 
\Note{otherwise} A naive approach, N is a constant known to the attacker; 
The attacker may use techniques such sequence slicing ... divide her inference scope... into per op and narrow down. Reduce the difficulty of inference (can we show that??)

Figure~\ref{fig:workflow} shows the case -- 
the attacker is uncertain the observed file trace consists of four amplified streams. 

\textbf{What about timing of amplification?}
\Note{needs more thoughts}
The obfuscator injects amplified stream without additional delay.
\Note{throttle the follow of the sybil ops??}
From the OS's perspective, the stream flows out back to back.
Due to the partitioned storage stack, the measurable execution time of each observed file op is unrelated to that of an actual op and is only subject to its resultant metadata disk requests which we will discuss in great detail in Section~\ref{sec:disk}.
Hence by measuring their execution time, an attacker cannot tell whether an op is actual/sybil and the number of amplifications.
 
\subsubsection{Horizontal amplification}

\Note{basically against differential analysis...}
homogenize the view of multiple \fs{}s as much as possible. 
reduce the attack surface of differential analysis. 

Why? all \fs{}s receive same transparent ops. Just non-transparent ops are different. 

With vertical amplification and the assembled sybil ops, the obfuscator finally fabricates them horizontally to the sybil \fs{}s.
 The challenge is how to make the horizontally amplified file trace appear indistinguishable from that on an actual \fs{}, so that it does not give away the identity of the sybil \fs{}.
 The identity of sybil \fs{}s is crucial since the obfuscator relies on them to protect non-transparent actual ops.
 Our rationale is: do nothing special unless necessary.
 
 
\paragraph{Rule V. Replicate transparent ops at all times}
\Note{useful message - all traces seem same transparent ops. 
leaving no basis for differential analysis}
The obfuscator does nothing special to \textit{hide} a sybil \fs{}.
Instead, it resembles an actual \fs{} by always replicating all transparent ops to sybil \fs{}s (as has been forecast in \S~\ref{sec:obfuscation:overall}, obfuscation step 3), including their types and arguments.
\Note{Seemingly naive but makes sense}
For files, it maps the ones in the vertical stream to those with same directory topology in sybil \fs{}s.
Since all \fs{}s have the same directory topology, it is always feasible to find such mapping.

\paragraph{Rule VI. Inject non-transparent ops as actual ops do}
As sybil \fs{}s are necessitated by protection of  actual non-transparent ops, they provide such protection only when needed, that is, an actual one is being amplified.
Hence, during horizontal amplification, the obfuscator does not inject non-transparent ops as ``freely'' as transparent ops; 
instead, it only assembles and injects non-transparent op to sybil \fs{}s when an actual non-transparent op.

\Note{This?}
For transparency, the actual fs cannot receive sybil non-transparent ops; for homogeneity, a sybil \fs{} shall receive the same amount of non-transparent ops as the actual fs. 

\Note{non-transparent ops will appear on all traces}
admit: the number of non-transparent ops exposed. 
but that's a design tradeoff we have to make. 
We add that to the public knowledge of $O$. see later section. 






==> obfuscator-op-generation-bak.tex <==










\section{Generating egalitarian sybil trace}
\label{sec:design:tracernr}

\input{fig-btt-ops}

\Note{this is 1st class question. should go up front}


\paragraph{Challenge: generating resembling noise}
For the sybil ops to be effective/deceptive, sybil ops must blend in well with actual ones without being identified.
Such task is challenging, because rich semantics exist not only within one file op itself but also across multiple ops.
Due to the challenge, naively drawing sybil ops with random arguments may break the invariants, which is easily identified by the OS.

For instance: open an non-existing files w/o O\_CREAT flag, read/write to a negative offset, etc.
More importantly, file ops are tied closely to the trustlet behavior, whose has a prescribed envelope of behavior.
For example, for an image recognition trustlet which always sequentially reads in the image, generating  a random sequences of reads do not make sense; 
for a database that reads in data from offsets depending on the query, always generating sequential reads does not make sense.











\subsection{Offline construction of trace library}

\Note{itemize as design objectives}

\Note{consider state: trustlets themselves have simpler control flow, e.g. as compared to smartphone apps. they are hence easier to exercise/test}

For resembling noise, \sys{} generates \textit{existing, real} file traces and inject them to sybil \fs{}s.
The rationale is the generated sybil ops are now fully immerse into the trustlet's envelopes of behaviors.
This justifies the ``similarity'' of synthesized behaviors on sybil \fs{}s with actual trustlet behaviors, such that an attacker cannot easily distinguish among actual and sybil file op streams.
Note that the goal is to discover what fs segments are \textit{possible}; we do not have to be exhaustive.

To build up the knowledge base of ``behaviors'', \sys{} fuzzes the trustlet and records its file traces (i.e. history) offline.
Ahead of time, offline testing: 
exercising trustlets in order to collect file traces. 
The goal of the test is to generate sufficiently diverse file traces; 
unlike bug finding or function validation, it does not have to be comprehensive and thorough. 
In practice, we find common software testing techniques adequate.

During offline testing, the fuzzer continuously fuzzes the trustlet function that results in interested file traces.
It uses structured fuzzing, which is well studied: depending on the trustlet category (\S\ref{sec:motiv:case}), it alters the input accordingly. 
For example, the fuzzer feeds different images to an image recognition trustlet;
for secure db, it feeds a variety of queries that respect the schema; the queries come from the test suite of the database.

Each input from the fuzzer leads to one file trace (although may not be unique), which is the \textbf{``atom''} for replaying -- the file trace will not be further split.
This is natural as the atom reflects one trustlet action.
Besides recording atoms, \sys{} also records the timings between file ops within an atom,
These all are stored and used for replaying on sybil \fs{}s.

\Note{storing the filetrace... could move to implementation (same nature as storing BTT)}
\sys{} uses an efficient data representation for storing them by exploiting the observation that many args are duplicate (e.g. read/write size): the atom contains only a sequence of file ops with args pointing to the argument pool. 
Should be highly compressible.
\sys{} stores the resultant trace library in normal world encrypted, appearing as a random binary blob to OS. 
\sys{} interacts with the library via normal file ops, whose file trace side-channel will be analyzed in \S\ref{sec:design:meta}.







\subsection{Online replay of sybil trace}

\Note{the ``stackable'' idea seems important. need to highlight.}
the more you need to hide (disguise), the higher risk you are in.

During trustlet execution, \sys{} generate resembling noise by replaying the atoms from the trace library offline recorded.

\Note{the model-based approach seems to contradict our own model-less principle}
\note{downplay the model-less principle}
\paragraph{Two stackable protection modes}
Targeting all three attack vectors (\S\ref{sec:motiv:case}), \sys{} features two stackable protection modes, namely timing and access pattern protection modes.
\begin{myenumerate}
	\item \textbf{Timing pattern}
	This mode protects timing pattern of trustlet (i.e. vector 1 in \S\ref{sec:motiv:case}).
	\sys{} instantiates timers for individual sybil \fs{}s for them to autonomously replay the recorded traces.
	\st{\sys{} exposes the API to trustlet for selecting well-known distributions (e.g. poisson distribution) to set up the timer.}
	The rationale is trustlets are event-driven, describable by stochastic process.
	At runtime, while replaying the recorded trace driven by sampling the timer distribution, \sys{} also continuously samples the arrival of actual events to calibrate the distribution. 
	This brings the timing of replayed sybil trace closer to the actual one.
	\item \textbf{File access pattern}
	The alternative mode, file access pattern mode protects secrets that lie in the inter/intra-file access pattern (attack vector 2 \& 3 in \S\ref{sec:motiv:case}) instead of their timings.
	Hence, there is no need to hide the actual trustlet file trace timing unless timing protection mode is enabled explicitly.
	The mode therefore replays the sybil file trace insync with the trustlet -- each time the trustlet issues actual file ops, \sys{} follows by replaying recorded sybil trace form the library.
\end{myenumerate}
	
Note that two modes are complementary to each other, thus stackable to mitigate attacks that exploits both timing and access pattern vectors, for instance, when the trustlet does not want the OS to know either the timing of a DB query or its content.

\paragraph{Replay unbounded stream of traces}
\sys{} ensures the replay of sybil traces never to exhaust by exploiting one insight: file traces are often recurring due to trustlet's behavior based on our case study, i.e. the trustlet keeps executing its mission loop.
Therefore, \sys{} draws traces from the trace library without deleting any to generate the unbounded stream of sybil trace for replaying, where one sybil trace may be replayed for multiple times in the long run.
Note that, during replay if new traces from the trustlet have been found it will be recorded...


\Note{not needed}
\paragraph{User APIs}
A manifest for developer to declare protection modes, and files.
For intra-file access pattern, it supplies single file. 
For inter-file access pattern, it supplies a directory.



















==> obliviousness.tex <==
\subsubsection{Oblivious block traces}

\input{fig-block-traces}

\note{this can go}

We experimentally demonstrate how obfuscation surface keeps \sys{} execution oblivious to an untrusted \fs{}. \note{always summarize result first}

In the experiment, a secure app opens a file and sequentially writes 256KB to it, where all each file operation are delegated to native \code{f2fs}, and \code{f2fs} protected by obfuscation surface with obfuscation level 5 and level 10, with respect to~Figure \ref{fig:block-traces} (a)-(c).
In each scenario, we run the experiment twice, reboot between runs to eliminate cache effects, and collect the block traces requested by the untrusted \fs{}.
As can be seen in Figure~\ref{fig:block-traces} (a), without obfuscation surface, the file operation delegated in two runs yield exactly same block traces observed by the untrusted \fs{}, which leads to access pattern exposure.
However, as demonstrated in~Figure \ref{fig:block-traces} (b) and (c), after the obfuscation surface, same delegated file operations yield two largely different block traces observed by an untrusted \fs{}.
As a result, an untrusted \fs{} cannot infer the access pattern of \sys{} or the directory structure of the file, because it is blinded as to which file operation is intended by \sys{}.



==> opt.tex <==

\section{Discussions}

Though without any optimizations, the overhead of waiting for the cloud verification is unaffordable, several optimizations are easily foreseeable.

\paragraph{Cached outcomes} 
A straightforward technique to reduce latency is to use cache.
Since each I/O request is a tuple containing $<blk\_no, page\_addr, len, offset>$,
each time such a message is sent to the cloud, a response can be cached in TEE and used later.

\paragraph{Evaluate block trustworthiness}
Current checkpoints will blindly checkpoint each write.
App can only access trusted block
Writes will update block status and invalidate trustworthiness until verified
Checkpoint existing content 








==> recycle-syscall-eg.tex <==

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstset{emph={%
	VALIDATION, O_UNTRUSTED%
	},emphstyle={\color{red}\bfseries}%
}%



\lstdefinestyle{mystyle}{
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

\lstset{style=mystyle}
\lstset{
xleftmargin=5.0ex,
framexleftmargin=5.0ex,
frame=tb, %
breaklines=true,
numberblanklines=false,
captionpos=b,
numbers=left,
label=list:api}
\begin{lstlisting}[caption= File trace observed by the attacker (i.e.\,an honest but curious OS). ,escapechar=!,label={code:syscall}]
open("nn_model.weights", O_RDONLY) = 3;
/* Loading conv layer1 */
read(3/*fd*/,0x2053340/*buf*/,0x1000 /*size*/);
read(3, 0x207511c, 0x11000);
read(3, 0x2053340, 0x1000);
/* Loading conv layer2 */
read(3, 0x2098f3c, 0x1000);
read(3, 0x2053340, 0x1000);
/* Loading conv layer3 */
read(3, 0x209cb5c, 0x11000);
read(3, 0x2053340, 0x1000);
...
open("captured_image", O_RDONLY) = 3;
/* Read JPEG-specific metadata */
pread64(3, 0x2053340, 0x1000, 0);
pread64(3, 0x2053340, 0x1000, 0xcd9);
pread64(3, 0x2053340, 0x1000, 0x2000);
...
/* A shiba inu doge has been detected */
open("detected_image", O_WRONLY|O_CREAT) = 3;
write(3, "...", 4096);
...
/* 15 sequential 4K writes */
...
write(3, "...", 1706);

\end{lstlisting}
\vspace{-1em}




==> sec-formulation.tex <==
\newpage
For any given input secret $s$, the observation by attacker is a sequence: 
\begin{equation}
	O(s) = (s_1, s_2, s_3, ..., s_k)
\end{equation}
Where $k$ is the total number of \fs{}. $s_k$ is the secret observed on $k$-th \fs{}; the secret $s$ hides in some $s_j, j\sim U[1,k]$.

Our goal is to prove for two distinct secrets given by trustlet $s_a$ and $s_b$, OS observes indistinguishable sequences.
This is formulated as the their probability difference (i.e. indistinguishablity as defined by k-anonymity, t-closeness..also used in path oram);
we prove the difference is bounded by a small constant $\delta$.
Equivalently, it is to prove:
\begin{equation}
	|Pr(O(s_a)) - Pr(O(s_b))| \leqslant \delta
\end{equation}
Where we have the following by Baysian law:
\begin{align}
	Pr(O(s_a)) & = Pr(s_1, s_2, ..., s_k)  \\
			 & = Pr(s_1, s_2, ..., s_{k-1} | s_a)Pr(s_a)
\end{align}
Since $s_a$ is already given, $s_k$ is independently sampled, we further have:
\begin{align}
	Pr(O(s_a)) &= \prod_{i=1}^{k-1}Pr(s_i)Pr(s_a) 
\end{align}

Hence we have
\begin{align}
	|Pr(O(s_a)) - Pr(O(s_b))| &= \prod_{i=1}^{k-1}Pr(s_i)|Pr(s_a) - Pr(s_b)| \\
							  &\leqslant \prod_{i=1}^{k-1}Pr(s_i) \\
							  &\leqslant \frac{1}{N^{k-1}} = \delta
\end{align}

For $N$ is the total number of secrets -- typically over 1000 (?); $k$ is the number of \fs{}s -- as large as 50. 
$\delta$ is hence as small as $10^{-100}$.
ORAM has similar formulation where $P=(\frac{1}{2^L})^M$. The P is comparable (XXX).

==> syscall-eg.tex <==

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstset{emph={%
	VALIDATION, O_UNTRUSTED%
	},emphstyle={\color{red}\bfseries}%
}%



\lstdefinestyle{mystyle}{
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

\lstset{style=mystyle}
\lstset{
xleftmargin=5.0ex,
framexleftmargin=5.0ex,
frame=tb, %
breaklines=true,
numberblanklines=false,
captionpos=b,
numbers=left,
label=list:eg1}
\begin{lstlisting}[escapechar=!,label={code:eg1}]
/* A: model file */
read(A, buf, !\Note{0x1000}!);
read(A, buf, !\Note{0x11000}!);
read(A, buf, !\Note{0x1000}!);
\end{lstlisting}




==> syscall-eg2.tex <==

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstset{emph={%
	VALIDATION, O_UNTRUSTED%
	},emphstyle={\color{red}\bfseries}%
}%



\lstdefinestyle{mystyle}{
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

\lstset{style=mystyle}
\lstset{
xleftmargin=5.0ex,
framexleftmargin=5.0ex,
frame=tb, %
breaklines=true,
numberblanklines=false,
captionpos=b,
numbers=left,
label=list:api}
\begin{lstlisting}[escapechar=!,label={code:eg2}]
if (detected) { 
	offset=get_file_offset(obj_id);
	write(fileA, offset ...); 
}
\end{lstlisting}




==> syscall-eg3.tex <==

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstset{emph={%
	VALIDATION, O_UNTRUSTED%
	},emphstyle={\color{red}\bfseries}%
}%



\lstdefinestyle{mystyle}{
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\fontsize{9}{9}\selectfont\ttfamily,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

\lstset{style=mystyle}
\lstset{
xleftmargin=5.0ex,
framexleftmargin=5.0ex,
frame=tb, %
breaklines=true,
numberblanklines=false,
captionpos=b,
numbers=left,
label=list:api}
\begin{lstlisting}[caption= The file trace of the trustlet writing out the detected object in a JPEG file. By observing the well-known offset the attacker infers a successful detection. ,escapechar=!,label={code:eg3}]
append(!\Note{secret}!);
append(!\Note{secret}! + 1024);
\end{lstlisting}
\vspace{-1em}




==> tab-2d.tex <==
\begin{table}[h]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/2d}
	\caption{Obfuscation featuring both shuffling and sybil files.XXX:place (1) on the left, pointing only to actual file}
\label{tab:2d}
\end{table}

==> tab-app-cases.tex <==

\begin{table}%
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/app-cases}
	\caption{	
	Trustlets and their file trace side channels
	}
	\label{tab:app-cases}
\end{table}


==> tab-cmp.tex <==
\begin{table}[t!]
	\fontsize{8.0}{9.0}\selectfont
	\begin{center}
		\setlength\tabcolsep{3pt}	%
		\begin{tabular}{
				l	%
				l	%
				l 	%
				c	%
				c	%
			}
			\hlineB{2.5}
			\cellcolor{lightgray}\textbf{System} &
			\cellcolor{lightgray}\textbf{TCB} & 
			\cellcolor{lightgray}\textbf{SG}
			\\ 
			\hlineB{1.5}
Cryptographic FS~\cite{cfs,ncryptfs,scfs} 				 	
& OS
& \texttt{CI-} \\ %


FS checkers~\cite{sqck,recon}
& OS
& \texttt{-I-} \\

Kernel checkers~\cite{sprobes,skee}
&  TEE
& \texttt{C$--$} \\

Outsource w/o verify~\cite{scone,graphene-sgx,obliviate,trustshadow}
& TEE
& \texttt{CI-} \\


\sys{} (this work)
& TEE
& \texttt{CIP} \\

\hlineB{2.5}
		\end{tabular}
		\fontsize{7.3}{7.7}\selectfont \\
		\textbf{SG}: security guarantees. \\ %
		\texttt{C}: data confidentiality; 
		\texttt{I}: data integrity; 
		\texttt{P}: persistence assurance\\
		\caption{A comparison of existing solutions and this work}
		\label{tab:cmp}
	\end{center}
\vspace{-2mm}
\end{table}

==> tab-file-ops.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Transparent ops & \code{read}, \code{write}, \code{stat} \\ \hline
Non-transparent ops & \code{append}, \code{create}, \code{delete}, \code{chmod}, \code{truncate}\\ \hline
\end{tabular}
\caption{Supported file ops}
\label{tab:fops}
\end{table}

==> tab-obfsucated-trace.tex <==

\begin{table}[]
\centering	
\includegraphics[width=0.48\textwidth]{figs/tab-obfuscated-trace}
\vspace*{-2em}
\caption{
	As obfuscation strength \K{} increases, it is increasingly difficult to recover the actual file trace from obfuscation.
	The actual ops marked in red.	
	For brevity, only op names are shown.
	Benchmark: \textbf{Video}.
}
\vspace*{-1em}
\label{tab:obfuscated-trace}
\end{table}

==> tab-obfuscate.tex <==
\begin{figure}[h!]%
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/eval-draft/tb}
	\caption{Is random guess better than DTW?}
	\label{fig:real}
\end{figure}


==> tab-rpc.tex <==
\begin{table}[h]
	\fontsize{8.0}{9.0}\selectfont
	\begin{center}
		\setlength\tabcolsep{3pt}	%
		\begin{tabular}{
				l   
				l	%
				l	%
				l	%
			}
			\hlineB{2.5}
			\textbf{ } &
			\textbf{100} &
			\textbf{100K} & 
			\textbf{1 Million}  
			\\ 
			\hlineB{1.5}
RPC cost				 	
& 100
& 10000
& 1000000\\

\hlineB{2.5}
		\end{tabular}
		\vspace{2mm}
		\caption{Time taken of RPC ping-pong, upon each SVC, TEE directly returns.}
		\vspace{-2mm}
		\label{tab:rpc}
	\end{center}
\end{table}

==> tab-sec-analysis.tex <==
\begin{table}[h]
	\fontsize{8.0}{9.0}\selectfont
	\begin{center}
		\setlength\tabcolsep{3pt}	%
		\begin{tabular}{
				l	%
				l	%
				l 	%
			}
			\hlineB{2.5}
			\textbf{Attack} &
			\textbf{Attack Vector} & 
			\textbf{Defense Mechanism} 
			\\ 
			\hlineB{1.5}

Syscall snooping
& File descriptor
& Secure VFS\\ 

PF/Cache
& File \& offset
& TEE Property\\



\hlineB{2.5}
		\end{tabular}
		\fontsize{7.3}{7.7}\selectfont \\
		\vspace{2mm}
		\caption{List of attacks and defense mechanisms of \sys{}. PF/Cache denotes page fault and cache based attack.
		}
		\label{tab:sec-analysis}
	\end{center}
\end{table}

==> tab-strawman-delay.tex <==
\begin{table}[h]
	\centering
	\includegraphics[page=1,width=0.48\textwidth{}]{./figs/tab_strawman_delay}
	\caption{File access delays of point solutions as comparisons}
	\label{tab:strawman:delay}
	\vspace*{-2em}
\end{table}


==> tab-strawman.tex <==
\begin{table*}[t]
	\centering
	\fontsize{7}{10}\selectfont
	\begin{tabular}{|l|l|l|l|l|l|l|}
	\hline

& IO Char                                                                & Dataset                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Access\\ latency\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Side\\ channels \end{tabular} & \begin{tabular}[c]{@{}l@{}}Sybil calls\\ \& emission\end{tabular}                          & Comparisons                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}\textbf{Database.} Query an on-device database of\\ user health data.\end{tabular}           & \begin{tabular}[c]{@{}l@{}}Single file,\\ rand RW\end{tabular}  & \begin{tabular}[c]{@{}l@{}}select[1-8] benchmarks from SQLite~\cite{sqlite-speedtest}. 
\\Total: 500 queries \\ 14K file calls. File size: 800KB\end{tabular}                                             & \begin{tabular}[c]{@{}l@{}}Per\\ query\end{tabular}              & \begin{tabular}[c]{@{}l@{}}Sizes/offsets\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}1 segments,  \\ 4-300 calls. \\ In sync \end{tabular} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} ORAM\end{tabular}} \\ \cline{1-6}
\begin{tabular}[c]{@{}l@{}}\textbf{Fulltext.} Search text files for on-device QA. \end{tabular}                        & \begin{tabular}[c]{@{}l@{}}Multi files,\\ rand RD\end{tabular} & \begin{tabular}[c]{@{}l@{}} Lucy~\cite{apache-lucy} on pre-indexed Enron emails~\cite{enron}.\\ Total: 100 queries; 100K file calls. File size: 2 GB\end{tabular} & \begin{tabular}[c]{@{}l@{}}Per\\ search\end{tabular}             & \begin{tabular}[c]{@{}l@{}}Sizes/offsets\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}1 segments,  \\ 1K calls \\ In sync \end{tabular}  &                                                                           \\ \cline{1-6}
\begin{tabular}[c]{@{}l@{}}\textbf{ModelLoad.}\\ Load ML models from files.\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Multi files,\\ rand RD\end{tabular} & \begin{tabular}[c]{@{}l@{}}TensorflowLite~\cite{tensorflow-web} loading 10 neural nets, \\ 80K file calls. File size: 41 MB.\end{tabular}                                                           & \begin{tabular}[c]{@{}l@{}}Load per\\ NN\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Sizes/offsets \\ File paths\end{tabular}       & \begin{tabular}[c]{@{}l@{}}1 segments,  \\ 8K calls \\ In sync \end{tabular}  &                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}\textbf{Historian.}\\ Log data bags from multiple sensors on a robot.\end{tabular}           & \begin{tabular}[c]{@{}l@{}}Single file, \\ Append\end{tabular}    & \begin{tabular}[c]{@{}l@{}} ROSbag on EU Long-term dataset~\cite{rosbag-data}.  \\ Total: 36K file calls.  File size: 659 MB.\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}Log per\\ data bag\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Sizes/offsets\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}1 segments,  \\ 1K calls \\ In sync \end{tabular}  & \begin{tabular}[c]{@{}l@{}}PadWrite\\-Only\end{tabular}                   \\ \hline
\begin{tabular}[c]{@{}l@{}}\textbf{VideoEv.}  Log images of motion events \\detected on a video stream.\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Multi files, \\ seq WR\end{tabular}     & \begin{tabular}[c]{@{}l@{}} 50 detected motion 1080P image frame on \\ Bangover video~\ref{bangover-data}. \\ 9K file calls. File size: 5MB\end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}Log per\\ image\end{tabular}          & Occurrence                                                                   & \begin{tabular}[c]{@{}l@{}}1 segments,  \\ 1 calls \\ out of sync\end{tabular}             & \begin{tabular}[c]{@{}l@{}} InjectCreate\\-Only\end{tabular}                 \\ \hline
\begin{tabular}[c]{@{}l@{}}\textbf{CredLoader.} Load credential files for \\ authentication with servers.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Multi file,\\ seq RD\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Load key files generated with ssh-keygen.\\ Total: 150 file calls. 50 files in 48KB.\end{tabular}                                           & \begin{tabular}[c]{@{}l@{}}Load per \\ key\end{tabular} & File paths                                                                   & \begin{tabular}[c]{@{}l@{}}1 segments,  \\ 3 calls \\ In sync \end{tabular}                 & \begin{tabular}[c]{@{}l@{}} InjectFiles\\-Only\end{tabular}                 \\ \hline

	\end{tabular}
	\caption{A summary of benchmarks}
	\label{tab:benchmarks}
\end{table*}


==> tab-tcb.tex <==
\begin{table}
\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/src}
	\caption{A comparison between the source of \sys{} and that of the Linux storage stack, showing that \sys{} reduces the on-device TCB significantly. \textbf{XXXX ext2?? Overwatch?? XXXX}}
	\label{tab:sloc}
\end{table}


==> tab-tracelet.tex <==
\begin{table}[h]
	\centering
	\includegraphics[width=0.5\textwidth{}]{./figs/tracelets}
	\caption{Tracelets and collection mechanism}
	\label{tab:tracelet}
\end{table}


==> todo.tex <==











\Note{Security}
\begin{myitemize}
	\item 
	Not considering integrity is a big problem. 
	Complementary efforts to integrity leaks information?
	\textbf{Revised in S2 \& S7.}
	
	\item 
	Unclear exactly which attacks can be thwarted. Never really define "which set of attacks the approach is truly able to thwart", clearer security model. More concrete attack examples. 
	"at least one compelling example of the premise of the problem"
	\textbf{Listed an attack example in S2.}

	\item 
	How does this model apply to Intel SGX, AMD SEV? More sound and detailed discussion. "Working only with TZ is a significant weakness". Comment about SGX confusing -- "why need Enigma when you already run a trusted VM"
	\textbf{Not a priority to fix}
	

	\item 
	Explain why ORAM might be a viable solution
	\textbf{Intro.}

	\item 
	What information can be extracted by attacker from replayed file ops? 
	\textbf{Revised in S5}


	
	\item 
	how is size of file handled? How are they hidden?
	\textbf{Not priority}

	\item 
	an attack: OS creates fingerprints FS by their unique metadata. Can't OS track individual FSes between FIDS intervals? 
	\textbf{Revised in S4}
	
	\item 
	How does TEE prevent OS from accessing the block device?
	\textbf{Revised in S6}

\end{myitemize}

\Note{FIDS..}
\begin{myitemize}
	\item 
	The chance of fses having same metadata accidentally? Shuffling always requires forking?
	Sensitivity analysis? 
	\textbf{Revised in S4.1}
	
	\item 
	Shuffle all both the actual \& sybil?
	\textbf{Revised in S4}
	
	\item 
	Can forking leak information? Can detecting forking help an attacker identify fs lineage? 
	\textbf{Revised in S4}

	
	\item 
	how is file creation/deletion tied to FIDS
	\textbf{Not priority}
	
	\item 
	Opened files during shuffling? 
	\textbf{Not priority}
	
	\item 
	Why is "several seconds" time window OK? "The reader has no way of knowing if several seconds of leaked history is dangerous or not" 
	\textbf{Added argument in S8}
	
	
\end{myitemize}

\Note{FSes \& Sybil Fses}
\begin{myitemize}
	\item 
	\sys{} makes the assumption that fs is large, complex while device drivers are small \& trivial to implement in TEE. When does the assumption hold? 
	\textbf{Not priority}

	\item 
	Understanding how file deletion \& creation works, how is file creation/deletion replicated
	\textbf{Not priority}
	
	\item 
	Does not have enough details of how record/replay works? E.g. unclear when \& how the file accesses are replayed. 
	\textbf{Existing in S5 but ignored}
	
	\item 
	How the developer feeds Enigma? 
	\textbf{Elaborate in S5}
	
	\item 
	The file ops are "randomly generated" that an attacker can infer which are invalid? 
	\textbf{Clarified in S5}
	
	\item 
	Do trustlets really need F2FS, EXT4? What hinders them is hardware limitation \& will be lifted (e.g. memory used to a problem for SGX but not anymore)? 
	\textbf{Reviewer misunderstands the work}
	
	\item 
	High runtime overhead -- unable to run more than 50 fses; should use way less 50 fses. 
	CPU usage high but never evaluated?
	\textbf{Reworded in S8}
	
	\item 
	Describe in more detail "the file calls in a segment are issued in a burst and their intervals ...'	
	\textbf{Sentence deleted}
\end{myitemize}


\Note{Impl. \& Eval}
\begin{myitemize}
	\item 
	How to read fig5-7 to compare point solutions \& baselines?
	No visual representation of ORAM results
	\textbf{The decision not to put baseline there was already discussed}
	
	\item 
	No FIO experiment evaluating fs perf on its own. 
	\textbf{Not priority}
	
	\item
	How do you have a 600LoC MMC driver?
	\textbf{Revised in S6}
	
	\item 
	BTT data structure? 
	\textbf{Not priority}
	
	\item 
	Clarify point solutions. "What are these exactly? Some non-security readers might lack this"
	\textbf{Revised in S8.1 tables \& comparisons}
	
	\item 
	Tone down the 1\% performance number. 
	\textbf{Revised abs.}
	
	\item 
	Why does security analysis come after Impl?
	\textbf{Not priority}
	

\end{myitemize}

\Note{Misc}
\textbf{Not priority}
\begin{myitemize}
	\item 
	Naming Enigma may be confusing because it refers to the encryption system at WWII
	
	\item 
	"trusted VM on the same machine disk hardware for the enclave" unclear about the SGX discussion. 
	
\end{myitemize}


==> trace-obfuscation.tex <==
\section{Trace Obfuscation}
\label{sec:design:obfuscator}

\Note{after extracting the key ideas to s4, do we still have substantial leftover? move to impl?}

The obfuscator (\circled{1}) sits between the trustlet and the normal world.
It works on \K{} files instead of one actual user file;
it obfuscates the actual file op of a trustlet to form \K{} sequences of file ops, bound to \K{} files;
it then forwards all sequences to normal world OS for execution.
We next describe the obfuscator design in detail.





\subsection{Design principles}


\paragraph{Our goals.}
We aim at a plausible solution by applying \K{}-anonymity to our problem domain: 
for the actual file ops that are inevitable to be revealed to normal world OS for execution (\S~\ref{sec:overview:idea}), we reduce the chance of the attacker ``guessing'' correctly the actual file and its respective file op arguments to $\frac{1}{\K{}}$;
for the overall actual file trace, we obfuscate it such that it is computationally difficult for the attacker to uncover. 

\Note{the following needs rethinking.}
\sys{} targets \textit{plausible} instead of \textit{proper} traces.
The arguments of sybil ops must appear \textit{similar} to the trustlet (by imitation).

	


\paragraph{Non-goals.} 
We do not aim to generate an obfuscated trace such that it appears \textit{proper} (to an adversarial observer), due to the lack of a holy grail specification in defining each program.
For example, a trustlet's file trace \code{open(fd), close(fd), write(fd,...)} can be regarded ``buggy'' due to it tries to write to a closed file.
However, defining it \textit{improper} and correcting it (i.e., to \code{open, write, close}) in the obfuscated trace is undesirable, as it fails the design objective (i.e., respecting trustlet's file ops) and digresses from the focus of this work.
\Note{this is interesting though. the attacker knows some ``impossible'' trace? see below.}

\Note{maybe still fold it into some desc}

this can be put under our framework.
we only ensure each op is feasible so the attacker cannot rule it out as actual op. 
we do not have to ensure the whole trace feasibility (and what is this?)
because even an infeasible trace observed by attacker may be amplified from a feasible actual trace. 
Again, this boils down to the whole set of fs behaviors; and the invariants that the attacker can use. 





\paragraph{Design choices}
To balance design goals and security requirements, the obfuscator follows design principles below.

\begin{myitemize}
	
	\item It adopts a \K{}-anonymity approach to hide the arguments of file ops needed to be disclosed for execution (e.g., which file to read/write, change of file permission) \Note{itemize them}.
	
	\item It works on a POSIX interface \Note{why say this?}. 
	It respects the actual file ops made by the trustlet.
	It does not shuffle data in file or directory namespaces.
	

	
	\item It generates \textit{plausible} instead of \textit{proper} traces.
	The arguments of sybil ops must appear \textit{similar} to the trustlet (by imitation).
	We will describe how shortly.
	\Note{no longer need this}
	
	\item It must obfuscate deterministically, so that by observing the same code run multiple times, the attacker sees same consistent (obfuscated) ones.	\Note{moved up}
	
	
	
	
\end{myitemize}











\subsection{Obfuscating a single file op?}
\label{sec:design:obfuscator}

\Note{a better sec name? does not sound new. why highlight?}

\paragraph{Key ideas.}
In applying the above principles to generate plausible yet deterministic obfuscated file trace, our key insights are to 1) use one-way secure hash function to guide the generation decisions (types, indexes, etc.), and 2) generate their arguments by imitating those of an actual file op from history. 

On one hand, hash functions, such as \code{SHA256}, produce unique digital fingerprint for different objects (e.g., binaries, messages); it is analogous to our scenario where we need to produce different obfuscated file traces for unique actual file ops.
On the other hand, by learning from the history of a trustlet's actual file ops, we eschew from reasoning about a \textit{proper} behavior on a per-trustlet basis.
We next formulate the problem and describe our approach.



\paragraph{Problem formulation.}
We first define a file op:
\begin{myitemize}
	\item \textit{File op}: a file op $f_n(x, args)$ is identified by the type (e.g., \code{read}, \code{write}, \code{fstat}), subject of the op (i.e., file descriptor $x$), the index $n$ in the sequence (i.e., memory address \Note{??}), and its respective arguments $args$ (offset, etc.).
\end{myitemize}
We seek to generate an obfuscated file trace:
\begin{myitemize}
	\item \textit{Obfuscated file trace}:given a file op $f_n(x, args)$ and obfuscation strength \K{}, an obfuscated file trace is a sequence of file ops, defined by \textbf{$F(x) = \{f'_{1}, ..., f'_{m}, ..., f'_{k} \}$}, where $f'_{m}$ is the same as $f_n(x,args)$ in type and $args$ if $x$ is an actual user file, otherwise ($x$ is a sybil file), $f'_{m}$ only has the same type as $f_n$, and $f'_{j} (j \neq m)$ is the injected normal op (i.e., sybil ops).
	\Note{too verbose}
\end{myitemize}

As can be seen, in generating the above obfuscated file trace, we need to answer two key questions:

\paragraph{Q1: How to decide the index $m$ of actual file op $f'_m$ and the injected normal ops $f'_{j}$?}
\Note{unnecessary}
Given an actual file op $f_i(x, args)$, the obfuscator uses its subject ($x$) and address ($i$) as inputs (i.e, as a message) to a hash function to generate a unique signature (i.e., the message digest).
The signature is a byte stream; 
by iterating through it, the obfuscator then decides the sybil ops $f'_{j}$ and the index $m$.
The process is straightforward: 
1) it finds $m$ by modding the whole byte stream by obfuscation strength \K{}; 
2) it decides $f'_{j}$ by iterating through the \K{} - 1 bytes and modding the current byte by total number of normal ops it sees to decide which normal op to inject \Note{type??}.
Note that for each sybil file $x'$ of the above actual file $x$, we will repeat the process 1) -- 2) to generate a respective obfuscated file IO, which is conceptually different than that of $x$ due to input of the hash function has changed to $x'$.







\paragraph{Q2: How to fill \textit{plausible} $args$ of sybil ops?}
In short, the generated arguments \textit{imitate} the historical ones from the actual file ops.
\Note{why do we do so?}
Similar to the process described above, the obfuscator collects the arguments it has seen for the \textbf{same} type of operations by far.
It selects the one by querying generated signature mod total number of arguments (as an index).
Although we refrain from reasoning about how to generate arguments for a \textit{proper} program behaviors in general due to lack of specifications, we find nevertheless our benchmarks all read within its file size \Note{???}.
Hence, in filling arguments (i.e., size) of read, we maintain an invariant that the read size does not exceed current file size.








\subsection{Sybil files: keep user files \K{}-anonymous}

\Note{copied upward}
\paragraph{Why \files{}?}
To hide the meta ops of the actual file op by bearing same type of meta ops with different arguments.
As explained in \S~\ref{sec:overview:idea}, we respect meta ops and forward them as-is to the actual user file.
If left unprotected (i.e., replicate the same meta ops with same arguments to \files{}), their arguments are leaked to the attacker, failing our design goals.
With \files{}, we hide the arguments of the actual meta ops by filling different arguments into \K{} - 1 extra meta ops (\S~\ref{sec:design:obfuscator}, $Q$2) destined to them, making it hard for the attacker to infer the actual arguments, which achieves our design goals.

\paragraph{What are \files{}?}
As has been forecast, they are the \K{}-anonymous instances of an actual user file.
For each actual user file, there exist \K{} - 1 sybil files.
Together they form a group \K{} files to bear the file ops issued by the obfuscator.



\paragraph{Lifecycle of \files{}.}
Upon the creation of each actual user file (i.e., \code{open} with \code{O\_CREAT}) , \K{} - 1 \files{} will also be created.
Their paths are deterministically generated:
similar to deciding sybil ops (\S~\ref{sec:design:obfuscator}, $Q$1), \sys{} hashes the actual user file name and samples the digest to iteratively generate the path as well as the sybil file names.
It is worth noting that the actual user file names received by the normal world OS are encrypted at the \tz{} boundary, hence both the names of the actual user file and its \files{} do not leak information.
After being created, \files{} will be opened/closed in sync with the actual user file and ops are applied to them, as mandated by the obfuscator.
When the actual user file is to be deleted (i.e., on a \code{unlinkat}), the \files{} will also be deleted.



\subsection{Limitations}

\note{At system design time, no app-specific behavior is taken into consideration.}
For example, a HMM can be defined and used to describe probable behaviors in terms of one syscall is more likely to happen than another.

Two aspects may prevent \sys{} from achieving full \K{}-anonymity.
First, despite the sybil ops and files, our technique still forwards the \textit{actual} file ops as requested, which is fundamental.
Hence, an attacker with \textit{enough} priori may rule out sybil ops and files, leading to sub-\K{} anonymity.
Second, sampling sybil ops and arguments from history needs to go through a cold start phase, whose duration depends on the trustlet. 
Before it can provide \K{} meaningful different arguments, meta ops' arguments are sub-\K{} anonymous.

